Universality of Linearized Message Passing for Phase Retrieval with Structured Sensing Matrices

In the phase retrieval problem one seeks to recover an unknown $n$ dimensional signal vector $\mathbf{x}$ from $m$ measurements of the form $y_i = |(\mathbf{A} \mathbf{x})_i|$, where $\mathbf{A}$ denotes the sensing matrix. Many algorithms for this problem are based on approximate message passing. For these algorithms, it is known that if the sensing matrix $\mathbf{A}$ is generated by sub-sampling $n$ columns of a uniformly random (i.e., Haar distributed) orthogonal matrix, in the high dimensional asymptotic regime ($m,n \rightarrow \infty, n/m \rightarrow \kappa$), the dynamics of the algorithm are given by a deterministic recursion known as the state evolution. For a special class of linearized message-passing algorithms, we show that the state evolution is universal: it continues to hold even when $\mathbf{A}$ is generated by randomly sub-sampling columns of the Hadamard-Walsh matrix, provided the signal is drawn from a Gaussian prior.

==> arxiv final/appendices.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% APPENDIX-TRACE%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Lemmas \ref{lemma: trace_good_event} and \ref{lemma: continuity_trace}}
\label{appendix: free_probability_trace}

\subsection{Proof of Lemma \ref{lemma: trace_good_event}}

\begin{proof}[Proof of Lemma \ref{lemma: trace_good_event}]
Recall that, $\bm A \bm A^\UT = \bm U \bm B \bm U^\UT, \; \bm \Psi = \bm A \bm A^\UT - \E [\bm A \bm A^\UT | \bm U] =  \bm U (\bm B - \kappa \bm I_m) \bm U^\UT$ where $\bm B$ is a uniformly random $m \times m$ diagonal matrix with exactly $n$ entries set to $1$ and the remaining entries set to $0$. 
Using the concentration inequality of Lemma \ref{concentration}:
\begin{align}
   \P \left( | (\bm A \bm A^\UT)_{ij} - \E (\bm A \bm A^\UT)_{ij}| > \epsilon \;  \big| \; \bm U\right) & \leq  4 \exp\left( - \frac{\epsilon^2}{8m \|\bm U\|_\infty^4} \right), \label{eq: conc_1}.
\end{align}
Setting $\epsilon = \sqrt{32 \cdot m \cdot  \|\bm U\|_\infty^4 \cdot  \log(m)}$ in \eqref{eq: conc_1} we obtain,
\begin{align*}
     \P \left( | (\bm A \bm A^\UT)_{ij} - \E (\bm A \bm A^\UT)_{ij}| > \sqrt{32 \cdot m \cdot  \|\bm U\|_\infty^4 \cdot  \log(m)} \;  \big| \; \bm U\right) & \leq  \frac{4}{m^4}.
\end{align*}
 By a union bound, $\P(\mathcal{E}^c | \bm U) \leq 4/m^2 \rightarrow 0$. In order to prove the claim of the lemma for the subsampled Haar model, we first note that by Fact \ref{fact: concentration_sphere} we have,
\begin{align*}
    \P\left( |O_{ij}| > \sqrt{\frac{8\log(m)}{m}} \right) & \leq  \frac{2}{m^4}.
\end{align*}
By a union bound $\P(\|\bm O\|_\infty > \sqrt{8\log(m)/m}) \leq 2m^{-2}$. This gives us:
\begin{align*}
    \P\left( \left\{\|\bm O\|_\infty \leq \sqrt{\frac{8\log(m)}{m}} \right\} \cap \mathcal{E} \right) &\geq 1 - \P\left(\|\bm O\|_\infty > \sqrt{\frac{8\log(m)}{m}}\right) - \P(\mathcal{E}^c) \\
    & \geq 1 - \frac{2}{m^2} - \E \P(\mathcal{E}^c|\bm U) \\
    & \geq 1 - \frac{6}{m^2}.
\end{align*}
This concludes the proof of the lemma. 
\end{proof}
\subsection{Proof of Lemma \ref{lemma: continuity_trace}}
\begin{proof}[Proof of Lemma \ref{lemma: continuity_trace}] Consider any alternating product $\mathcal{A}$ (see Definition \ref{def: alternating_product}):
\begin{align*}
    \altprod(\bm \Psi,\bm Z) = (\bm \Psi) q_1(\bm Z) (\bm \Psi) \cdots  q_k(\bm Z).
\end{align*}
Note that in the above expression, we have assumed the alternating product is of Type 2 but the following argument applies to all the other types too. We define:
\begin{align*}
    \altprod_i & = (\bm \Psi) q_1(\bm Z) (\bm \Psi) q_2(\bm Z) \cdots (\bm \Psi) q_i(\bm Z) (\bm \Psi) q_{i+1}(\bm Z^\prime) (\bm \Psi) q_{i+2}(\bm Z^\prime) \cdots (\bm \Psi ) q_k(\bm Z^\prime).
\end{align*}
Then we can express $\altprod(\bm \Psi, \bm Z^\prime)  - \altprod(\bm \Psi, \bm Z) $ as a telescoping sum:
\begin{align*}
    \altprod(\bm \Psi, \bm Z)  - \altprod(\bm \Psi, \bm Z^\prime) & = \sum_{i=1}^k (\altprod_{i}-\altprod_{i-1}).
\end{align*}
Hence,
\begin{align*}
    \left| \frac{\Tr \altprod(\bm \Psi, \bm Z)}{m} - \frac{\Tr \altprod(\bm \Psi, \bm Z^\prime)}{m} \right| & \leq \frac{1}{m} \sum_{i=1}^k |\Tr(\altprod_i - \altprod_{i-1})|.
\end{align*}
Next we observe that:
\begin{align*}
    &|\Tr(\altprod_i - \altprod_{i-1})| \\& = |\Tr( (\bm \Psi) q_1(\bm Z) \cdots (\bm \Psi) q_{i-1}(\bm Z) \cdot (q_i(\bm Z) - q_{i}(\bm Z^\prime)) \cdot (\bm \Psi) q_{i+1}(\bm Z^\prime) \cdots (\bm \Psi) q_{k}(\bm Z^\prime))| \\
    & \leq \left\|(\bm \Psi) q_1(\bm Z) \cdots (\bm \Psi) q_{i-1}(\bm Z) \cdot  (\bm \Psi) q_{i+1}(\bm Z^\prime) \cdots (\bm \Psi) q_{k}(\bm Z^\prime) \right\|_\op \cdot \left( \sum_{j=1}^m |q_i(z_j) - q_i(z_j^\prime)| \right) \\
    & \leq \|(\bm \Psi)\|_{\op} \|q_1(\bm Z)\|_\op \cdots \| (\bm \Psi)\|_\op \| q_{k}(\bm Z^\prime)\|_\op \cdot \left( \sum_{j=1}^m |q_i(z_j) - q_i(z_j^\prime)| \right)\\
    & \explain{(a)}{\leq} \left(\prod_{j=1}^k \|q_j\|_\infty \right) \cdot \|q_i\|_{\mathsf{Lip}} \cdot \left( \sum_{j=1}^m |z_j - z_j^\prime| \right) \\
    & \leq \sqrt{m} \cdot C(\altprod) \cdot \|\bm Z- \bm Z^\prime\|_\fr. 
\end{align*}
In the step marked (a), we observed that: $\|(\bm \Psi)\|_{\op} = \|\bm U (\barB) \bm U^\UT\|_{\op} \leq \max(|\kappa)|, |1-\kappa|) \leq 1$. Similarly, $\|q_j(\bm Z)\|_{\op} \leq \|q_j\|_\infty \explain{def}{=} \sup_{\xi \in \R} |q_j(\xi)|$. We also recalled the functions $q_i$ are assumed to be Lipchitz and denoted the Lipchitz constant of $q_i$ by $\|q_i\|_{\mathsf{Lip}}$. Hence we obtain:
\begin{align*}
    \left| \frac{\Tr \altprod(\bm \Psi, \bm Z)}{m} - \frac{\Tr \altprod(\bm \Psi, \bm Z^\prime)}{m} \right| & \leq \frac{k \cdot  C(\altprod)}{\sqrt{m}} \cdot  \|\bm Z- \bm Z^\prime\|_\fr.
\end{align*}
This concludes the proof of the lemma.
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% APPENDIX-QF-VARIANCE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Proposition \ref{prop: qf_univ_mom2}}
\label{supplement: qf_univ_mom2}
The proof of Proposition \ref{prop: qf_univ_mom2} is very similar to the proof of Proposition \ref{prop: qf_univ_mom1} and hence we will be brief in our arguments. 

As discussed in the proof of Proposition \ref{prop: qf_univ_mom1}, we will assume that alternating form is of Type 1. The other types are handled as outlined in Remark \ref{remark: all_types_qf_mom1}. Furthermore, in light of Lemma \ref{lemma: poly_psi_simple} we can further assume that all polynomials $p_i(\psi) = \psi$. Hence we assume that $\altprod$ is of the form: $$\altprod(\bm \Psi, \bm Z) = \bm \Psi q_1(\bm Z)\bm \Psi \cdots  q_{k-1}(\bm Z) \bm \Psi.$$

The proof of Proposition \ref{prop: qf_univ_mom2} consists of various steps which will be organized as separate lemmas. We begin by recall that 
\begin{align*}
    \bm z & \sim \gauss{0}{\frac{\bm A \bm A^\UT}{\kappa}}.
\end{align*}
Define the event:
    \begin{align}
        \mathcal{E}  &= \left\{ \max_{i \neq j} | (\bm A \bm A^\UT|)_{ij} \leq \sqrt{\frac{2048 \cdot  \log^{3}(m)}{m}}, \; \max_{i \in [m]} | (\bm A \bm A^\UT)_{ii} - \kappa | \leq \sqrt{\frac{2048 \cdot  \log^{3}(m)}{m}} \right\} %\label{eq: good_event_qf_firstmom}
    \end{align}
    By Lemma \ref{lemma: trace_good_event} we know that $\P(\mathcal{E}^c) \rightarrow 0$ for both the subsampled Haar sensing and the subsampled Hadamard model. 
    We define the normalized random vector $\widetilde{\bm z}$ as:
\begin{align*}
    \widetilde{z}_i & = \frac{z_i}{\sigma_i}, \; \sigma_i^2 = \frac{(\bm A \bm A^\UT)_{ii}}{\kappa} %\label{eq: tilde_z_distribution}
\end{align*}
Note that conditional on $\bm A$, $\widetilde{\bm z}$ is a zero mean Gaussian vector with: $$\E[\widetilde{z_i}^2 | \bm A] =1, \; \E[ \widetilde{z}_i \widetilde{z_j} | \bm A] = \frac{(\bm A \bm A^\UT)_{ij}/\kappa}{\sigma_i \sigma_j}.$$ We define the diagonal matrix $\widetilde{\bm Z} = \diag{\widetilde{\bm z}}$.

\begin{lem}\label{lemma : qf_mom2_variance_normalization} We have, \begin{align*}
    \lim_{m \rightarrow \infty} \frac{\E (\bm z^\UT \altprod(\bm \Psi, \bm Z) \bm z)^2}{m^2}&=\lim_{m \rightarrow \infty} \frac{ \E(\widetilde{\bm z}^{\UT} \altprod(\bm\Psi, \widetilde{\bm Z}) \widetilde{\bm z})^2}{m^2} \Indicator{\mathcal{E}},
\end{align*}
provided the latter limit exists.
\end{lem}
The proof of this lemma is analogous the proof of Lemma \ref{lemma : qf_variance_normalization} and is omitted.   The advantage of Lemma \ref{lemma : qf_mom2_variance_normalization} is that $\widetilde{z}_i \sim \gauss{0}{1}$ and on the event $\mathcal{E}$ the coordinates of  $\widetilde{\bm z}$ have weak correlations. Consequently, Mehler's Formula (Proposition \ref{proposition: mehler}) can be used to analyze the leading order term in $\E[\widetilde{\bm z}^{\UT} \altprod(\bm\Psi, \widetilde{\bm Z}) \widetilde{\bm z} \;  \Indicator{\mathcal{E}}]$. Before we do so, we do one additional preprocessing step. 

\begin{lem}\label{lemma: qf_mom2_diagonal_removal} We have, 
\begin{align*}
    \lim_{m \rightarrow \infty} \frac{ \E(\widetilde{\bm z}^{\UT} \altprod(\bm\Psi, \widetilde{\bm Z}) \widetilde{\bm z})^2}{m^2} \Indicator{\mathcal{E}}&=\lim_{m \rightarrow \infty} \frac{\E \; \Tr (\altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT -  \widetilde{\bm Z}^2) \cdot \altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT -  \widetilde{\bm Z}^2)  ) \Indicator{\mathcal{E}}}{m^2},
\end{align*}
provided the latter limit exists. 
\end{lem}
\begin{proof}[Proof Sketch] Observe that we can write:
    \begin{align*}
        &(\widetilde{\bm z}^\UT \altprod \widetilde{\bm z})^2  =\Tr(\altprod \cdot \widetilde{\bm z} \widetilde{\bm z}^\UT \cdot \altprod \cdot \widetilde{\bm z} \widetilde{\bm z}^\UT)  \\
        & = \Tr(\altprod \cdot (\widetilde{\bm z}\widetilde{\bm z}^\UT -\widetilde{\bm Z}^2 + \widetilde{\bm Z}^2) \cdot \altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT-\widetilde{\bm Z}^2 + \widetilde{\bm Z}^2)) \\
        & = \Tr(\altprod \cdot (\widetilde{\bm z}\widetilde{\bm z}^\UT -\widetilde{\bm Z}^2) \cdot \altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT-\widetilde{\bm Z}^2)) + \Tr(\altprod \cdot  \widetilde{\bm Z}^2 \cdot \altprod \cdot \widetilde{\bm z} \widetilde{\bm z}^\UT) + \Tr(\altprod \cdot \widetilde{\bm z} \widetilde{\bm z}^\UT \cdot  \widetilde{\bm Z}^2 \cdot\altprod  )  \\& \hspace{6cm}- \Tr(\altprod \cdot \widetilde{\bm Z}^2  \cdot \altprod \cdot \widetilde{\bm Z}^2) \\
        & = \Tr(\altprod \cdot (\widetilde{\bm z}\widetilde{\bm z}^\UT -\widetilde{\bm Z}^2) \cdot \altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT-\widetilde{\bm Z}^2))  + 2 \widetilde{\bm z}^\UT\altprod \cdot  \widetilde{\bm Z}^2 \cdot \altprod \cdot \widetilde{\bm z} - \Tr(\altprod \cdot \widetilde{\bm Z}^2  \cdot \altprod \cdot \widetilde{\bm Z}^2).
    \end{align*}
    Next we note that:
    \begin{align*}
         |\widetilde{\bm z}^\UT\altprod \cdot  \widetilde{\bm Z}^2 \cdot \altprod \cdot \widetilde{\bm z}| & \leq \|\widetilde{\bm z}\|^2 \cdot \|\altprod\|_\op^2 \cdot \left( \max_{i \in [m]} |\widetilde{z}_i|^2 \right) \leq O_P(m) \cdot O(1) \cdot O_P(\polylog(m)),
    \end{align*}
    Hence it can be shown that,
    \begin{align*}
        \frac{\E |\widetilde{\bm z}^\UT\altprod \cdot  \widetilde{\bm Z}^2 \cdot \altprod \cdot \widetilde{\bm z}|}{m^2} \rightarrow 0.
    \end{align*}
    Similarly,
    \begin{align*}
        |\Tr(\altprod \cdot \widetilde{\bm Z}^2  \cdot \altprod \cdot \widetilde{\bm Z}^2)| & \leq m \|\altprod \cdot \widetilde{\bm Z}^2  \cdot \altprod \cdot \widetilde{\bm Z}^2\|_\op \leq m\|\altprod\|_\op^2 \cdot \left( \max_{i \in [m]} |\widetilde{z}_i|^4 \right)\\ &\leq O(m) \cdot O(1) \cdot O_P(\polylog(m)),
    \end{align*}
    and hence one expects that,
    \begin{align*}
        \frac{\E|\Tr(\altprod \cdot \widetilde{\bm Z}^2  \cdot \altprod \cdot \widetilde{\bm Z}^2)|}{m^2} \rightarrow 0.
    \end{align*}
    We omit the detailed arguments. This concludes the proof of the lemma.
\end{proof}
Note that, so far, we have shown that:
\begin{align*}
       \lim_{m \rightarrow \infty} \frac{\E (\bm z^\UT \altprod(\bm \Psi, \bm Z) \bm z)^2}{m^2}&=\lim_{m \rightarrow \infty}\frac{\E \; \Tr (\altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT -  \widetilde{\bm Z}^2) \cdot \altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT -  \widetilde{\bm Z}^2)  ) \Indicator{\mathcal{E}}}{m^2},
\end{align*}
provided the latter limit exists. We now focus on analyzing the RHS. We expand 
    \begin{align*}
        & \; \Tr (\altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT -  \widetilde{\bm Z}^2) \cdot \altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT -  \widetilde{\bm Z}^2)  ) = \\& \sum_{\substack{a_{1:2k+2} \in [m]\\ a_1 \neq a_{2k+2}\\ a_{k+1} \neq a_{k+2}}}  (\bm \Psi)_{a_1,a_2} q_1(\widetilde{z}_{a_2}) \cdots  (\bm \Psi)_{a_k,a_{k+1}} \widetilde{z}_{a_{k+1}} \widetilde{z}_{a_{k+2}} (\bm \Psi)_{a_{k+2},a_{k+3}} q_1(\widetilde{z}_{a_{k+3}})  \cdots   (\bm \Psi)_{a_{2k+1},a_{2k+2}} \widetilde{z}_{a_{2k+2}} \widetilde{z}_{a_1}.
    \end{align*}
    This can be written compactly in terms of matrix moments (Definition \ref{def: matrix moment}) as follows: Let $\dlgraph \in \weightedG{2k+2}$ denote the graph formed by combining two disconnected copies of the simple line graph on vertices $[1:k+1]$ and $[k+2: 2k +2]$:
    \begin{align*}
        (\dlgraph)_{ij} & = \begin{cases} 1 : & |i-j| = 1, \; \{i,j\} \neq \{k+1,k+2\}, \\ 0 : &\text{otherwise} \end{cases}.
    \end{align*}
    Recall the notation for partitions introduced in Section \ref{section: partition_notation}. Observe that:
    \begin{align*}
        \{(a_1 \dots a_{2k+2}) \in [m]^{2k+2} : \; a_1 \neq a_{2k+2}, \; a_{k+1} \neq a_{k+2} \} & = \bigsqcup_{\pi \in \part{0}{[2k+2]}}  \cset{\pi},
    \end{align*}
    where,
    \begin{align*}
        \part{0}{[2k+2]} &\explain{def}{=} \{\pi \in \part{}{2k+2}: \pi(1) \neq \pi(2k+2), \; \pi(k+1) \neq \pi(k+2)\}.
    \end{align*}
    Recalling Definition \ref{def: matrix moment}, we have,
    \begin{align*}
        (\bm \Psi)_{a_1,a_2} \cdots (\bm \Psi)_{a_k,a_{k+1}} (\bm \Psi)_{a_{k+2},a_{k+3}}   \cdots   (\bm \Psi)_{a_{2k+1},a_{2k+2}} & = \matmom{\bm \Psi}{\dlgraph}{\pi}{\bm a}
    \end{align*}
    Hence,
    \begin{align*}
        &\frac{\E \; \Tr (\altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT -  \widetilde{\bm Z}^2) \cdot \altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT -  \widetilde{\bm Z}^2)  ) \Indicator{\mathcal{E}}}{m^2} = \\& \hspace{0cm} \frac{1}{m^2} \sum_{\substack{\pi \in \part{0}{2k+2}\\ \bm a \in \cset{\pi}}} \E \; \matmom{\bm \Psi}{\dlgraph}{\pi}{\bm a}  \cdot(\widetilde{z}_{a_1} q_1(\widetilde{z}_{a_2}) \cdots    \widetilde{z}_{a_{k+1}} \widetilde{z}_{a_{k+2}}  q_1(\widetilde{z}_{a_{k+3}})  \cdots   \widetilde{z}_{a_{2k+2}}) \cdot  \Indicator{\mathcal{E}}.
    \end{align*}
    By the tower property,
 \begin{align*}
        &\E \; \matmom{\bm \Psi}{\dlgraph}{\pi}{\bm a}  \cdot(\widetilde{z}_{a_1} q_1(\widetilde{z}_{a_2}) \cdots    \widetilde{z}_{a_{k+1}} \widetilde{z}_{a_{k+2}}  q_1(\widetilde{z}_{a_{k+3}})  \cdots   \widetilde{z}_{a_{2k+2}}) \cdot  \Indicator{\mathcal{E}} =  \\&\hspace{1cm}\E \left[ \matmom{\bm \Psi}{\dlgraph}{\pi}{\bm a}  \cdot\E[ \widetilde{z}_{a_1} q_1(\widetilde{z}_{a_2}) \cdots    \widetilde{z}_{a_{k+1}} \widetilde{z}_{a_{k+2}}  q_1(\widetilde{z}_{a_{k+3}})  \cdots   \widetilde{z}_{a_{2k+2}} |  \bm A ] \Indicator{\mathcal{E}} \right].
    \end{align*}
    We will now use Mehler's formula (Proposition \ref{proposition: mehler}) to evaluate $\E[ \cdots |  \bm A ]$ upto leading order. Note that some of the random variables $\widetilde{z}_{a_{1:2k+2}}$ are equal (as given by the partition $\pi$). Hence we group them together and recenter the resulting functions. The blocks corresponding to $a_1, a_{k+1},a_{k+2},a_{2k+2}$ need to be treated specially due to the presence of $\widetilde{z}_{a_1},\widetilde{z}_{a_{k+1}},\widetilde{z}_{a_{k+2}}, \widetilde{z}_{a_{2k+2}}$ in the above expectations. Hence, we introduce the following notations:
     We introduce the following notations:
    \begin{align*}
        \fblknum{1}{\pi} & = \pi(1), \; \lblknum{1}{\pi}= \pi(k+1), \; \fblknum{2}{\pi}= \pi(k+2), \; \lblknum{2}{\pi} = \pi(2k+2)  \\ \singleblks{\pi} &= \{i \in [1:2k+2]\backslash \{1,k+1,k+2,2k+2\}: |\pi(i)| = 1 \}.
    \end{align*}
    We label all the remaining blocks of $\pi$ as $\blocks_1,\blocks_2 \dots \blocks_{|\pi| - |\singleblks{\pi}| - 4}$. Hence the partition $\pi$ is given by:
    \begin{align*}
        \pi = \fblknum{1}{\pi} \sqcup \lblknum{1}{\pi} \sqcup \fblknum{2}{\pi} \sqcup \lblknum{2}{\pi} \sqcup \left( \bigsqcup_{i \in \singleblks{\pi}} \{i\} \right) \sqcup \left( \bigsqcup_{t=1}^{|\pi| - |\singleblks{\pi}| - 4} \blocks_i\right).
    \end{align*}
    To simplify notation, we additionally define:
    \begin{align*}
        q_{k+1 + i}(\xi) \explain{def}{=} q_{i}(\xi), \; i = 1,2 \dots k-1.
    \end{align*}
    Note that: 
    \begin{align*}
        &\widetilde{z}_{a_1} \widetilde{z}_{a_{k+1}}\widetilde{z}_{a_{k+2}}\widetilde{z}_{a_{2k+2}}\prod_{\substack{i=1\\ i \neq k,k+1}}^{2k} q_i(\widetilde{z}_{a_{i+1}})  = \\& Q_\ffncnum{1}(\widetilde{z}_{a_1})  Q_\lfncnum{1}(\widetilde{z}_{a_{k+1}})  Q_\ffncnum{2}(\widetilde{z}_{a_{k+2}})   Q_\lfncnum{2}(\widetilde{z}_{a_{2k+2}}) \left( \prod_{i \in \singleblks{\pi}} q_{i-1}(\widetilde{z}_{a_i}) \right)  \prod_{i=1}^{|\pi| - |\singleblks{\pi}| - 4} (Q_{\blocks_i}(z_{a_{\blocks_i}}) + \mu_{\blocks_i}),
    \end{align*}
    where,
    \begin{align*}
        Q_\ffncnum{1}(\xi) & = \xi \cdot \prod_{i \in \fblknum{1}{\pi}, i \neq 1} q_{i-1}(\xi), \\
        Q_\lfncnum{1}(\xi) & = \xi \cdot \prod_{i \in \lblknum{1}{\pi}, i \neq k+1} q_{i-1}(\xi), \\
        Q_\ffncnum{2}(\xi) & = \xi \cdot \prod_{i \in \fblknum{2}{\pi}, i \neq k+2} q_{i-1}(\xi), \\
        Q_\lfncnum{2}(\xi) & = \xi \cdot \prod_{i \in \lblknum{2}{\pi}, i \neq 2k+2} q_{i-1}(\xi), \\
        \mu_{\blocks_i} & = \E_{\xi \sim \gauss{0}{1}} \left[ \prod_{j \in \blocks_i} q_{j-1}(\xi) \right], \\
        Q_{\blocks_i}(\xi) & = \prod_{j \in \blocks_i} q_{j-1}(\xi) - \mu_{\blocks_i}, \\
    \end{align*}
     With this notation in place we can apply Mehler's formula. The result is summarized in the following lemma.
     \begin{lem} \label{lemma: qf_mehler_conclusion_mom2} For any $\pi \in \part{0}{[2k+2]}$ and any $\bm a \in \cset{\pi}$ we have,
\begin{subequations}
    \begin{align*}
        &\Indicator{\mathcal{E}}  \left| \E[ \widetilde{z}_{a_1} q_1(\widetilde{z}_{a_2}) \cdots    \widetilde{z}_{a_{k+1}} \widetilde{z}_{a_{k+2}}  q_1(\widetilde{z}_{a_{k+3}})  \cdots  \widetilde{z}_{a_{2k+2}} |  \bm A ] - \sum_{\bm w \in \weightedGnum{\pi}{2}} {\Coeff}(\bm w, \pi) \cdot \matmom{\bm \Psi}{\bm w}{\pi}{\bm a}  \right| \nonumber \\
             &\hspace{8cm }  \leq C(\altprod) \cdot \left( \frac{\log^3(m)}{m \kappa^2} \right)^{\frac{3 + |\singleblks{\pi}|}{2}},
    \end{align*}
    where, $\matmom{\bm \Psi}{\bm w}{\pi}{\bm a}$ is the matrix moment as defined in Definition \ref{def: matrix moment}, 
    \begin{align*}
        {\Coeff}(\bm w, \pi) & = \frac{1}{{\kappa^{\|\bm w\|}} \bm w!}   \left(\hat{Q}_\ffncnum{1}(1) \hat{Q}_\lfncnum{1}(1) \hat{Q}_\ffncnum{2}(1)\hat{Q}_\lfncnum{2}(1) \prod_{i \in \singleblks{\pi}} \hat{q}_{i-1}(2)   \right)   \left( \prod_{i \in [|\pi| - |\singleblks{\pi}| - 4]} \mu_{\blocks_i} \right)
    \end{align*}
    \begin{align*}
            \weightedGnum{\pi}{2} & \explain{def}{=} \left\{\bm w \in \weightedG{2k+2}: \degree_i(\bm w) = 1 \; \forall \; i \; \in \; \{1,k+1,k+2,2k+2\}, \right. \nonumber\\ &\hspace{1cm} \degree_i(\bm w) = 2 \; \forall \; i \; \in \; \singleblks{\pi},  \left.\degree_i(\bm w) = 0 \; \forall \; i \; \notin \; \{1,k+1,k+2,2k+2\} \cup \singleblks{\pi} \right\},
        \end{align*}
    %\label{eq: mehler_conclusion_imp}
    \end{subequations}
     \end{lem}
The proof of the lemma involves instantiating Mehler's formula for this situation and identifying the leading order term. Since the proof is analogous to the proof of Lemma \ref{lemma: qf_mehler_conclusion} provided in Appendix \ref{proof: qf_mehler_conclusion}, we omit it.

We return to our analysis of:
\begin{align*}
        &\frac{\E \; \Tr (\altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT -  \widetilde{\bm Z}^2) \cdot \altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT -  \widetilde{\bm Z}^2)  ) \Indicator{\mathcal{E}}}{m^2} = \\& \hspace{0cm} \frac{1}{m^2} \sum_{\substack{\pi \in \part{0}{2k+2}\\\bm a \in \cset{\pi}}} \E \; \matmom{\bm \Psi}{\dlgraph}{\pi}{\bm a}  \cdot(\widetilde{z}_{a_1} q_1(\widetilde{z}_{a_2}) \cdots    \widetilde{z}_{a_{k+1}} \widetilde{z}_{a_{k+2}}  q_1(\widetilde{z}_{a_{k+3}})  \cdots   \widetilde{z}_{a_{2k+2}}) \cdot  \Indicator{\mathcal{E}}.
\end{align*}
We define the following  subsets of $\part{0}{2k+2}$ as:
\begin{subequations}
\label{eq: qf_firstmom_goodpartitions_mom2}
\begin{align}
    \part{1}{[2k+2]} & \explain{def}{=} \left\{\pi \in \part{0}{2k+2
    }: \; |\pi(i)| = 1, \; \forall \; i \; \in \; \{1,k+1,k+2,2k+2\},\right. \\ \nonumber&\left. \hspace{8cm} |\pi(j)| \leq 2 \; \forall \; j \; \in \; [k+1]\right\}, \\
    \part{2}{[2k+2]} & \explain{def}{=} \part{0}{[2k+2]} \backslash \part{1}{[2k+2]},
\end{align}
\end{subequations}
and the error term which was controlled in Lemma \ref{lemma: qf_mehler_conclusion}:
\begin{align*}
        &\epsilon(\bm \Psi, \bm a) \explain{def}{=}\\& \Indicator{\mathcal{E}}  \left( \E[ \widetilde{z}_{a_1} q_1(\widetilde{z}_{a_2}) \cdots    \widetilde{z}_{a_{k+1}} \widetilde{z}_{a_{k+2}}  q_1(\widetilde{z}_{a_{k+3}})  \cdots   \widetilde{z}_{a_{2k+2}} |  \bm A ] - \sum_{\bm w \in \weightedGnum{\pi}{2}} {\Coeff}(\bm w, \pi) \cdot \matmom{\bm \Psi}{\bm w}{\pi}{\bm a}  \right)\end{align*}.

With these definitions we consider the decomposition:
\begin{align*}
    &\frac{\E \; \Tr (\altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT -  \widetilde{\bm Z}^2) \cdot \altprod \cdot (\widetilde{\bm z} \widetilde{\bm z}^\UT -  \widetilde{\bm Z}^2)  ) \Indicator{\mathcal{E}}}{m^2} = \\& \hspace{1cm} \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{a \in \cset{\pi}} \sum_{\bm w \in \weightedGnum{\pi}{2}} {\Coeff}(\bm w, \pi) \cdot \E\left[\matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right] - \mathsf{I} + \mathsf{II} + \mathsf{III},
\end{align*}
where, 
\begin{align*}
    \mathsf{I} &\explain{}{=}\frac{1}{m^2} \sum_{\substack{\pi \in \part{0}{[2k+2]}}}\sum_{a \in \cset{\pi}} \sum_{\bm w \in \weightedGnum{\pi}{2}} {\Coeff}(\bm w, \pi) \cdot \E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \Indicator{\mathcal{E}^c} \right], \\
    \mathsf{II} & = \frac{1}{m^2} \sum_{\pi \in \part{0}{2k+2]}} \sum_{a \in \cset{\pi}} \E\left[   \matmom{\bm \Psi}{\dlgraph}{\pi}{\bm a}\epsilon(\bm \Psi, \bm a) \Indicator{\mathcal{E}} \right], \\
     \mathsf{III} & \explain{}{=} \frac{1}{m^2} \sum_{\pi \in \part{2}{[2k+2]}} \sum_{a \in \cset{\pi}} \sum_{\bm w \in \weightedGnum{\pi}{2}} {\Coeff}(\bm w, \pi) \cdot \E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right].
\end{align*}
We will show that $\mathsf{I}, \mathsf{II}, \mathsf{III} \rightarrow 0$. Showing this involves the following components:
\begin{enumerate}
    \item Bounds on matrix moments $\E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right]$ which have been developed in Lemma \ref{lemma: matrix_moment_ub}. 
    \item Controlling the size of the set $|\cset{\pi}|$ (since we sum over $\bm a \in \cset{\pi}$ in the above terms). Since, 
    \begin{align*}
        |\cset{\pi}| & = m(m-1) \cdots (m-|\pi| + 1) \asymp m^{|\pi|},
    \end{align*}
    we need to develop bounds on $|\pi|$. This is done in the following lemma. In contrast, the sums over $\pi \in \part{0}{[2k+2]}$ and $\bm w \in \weightedGnum{\pi}{1}$ are not a cause of concern since $|\part{0}{[2k+2]}|,|\weightedGnum{\pi}{1}|$ depend only on $k$ (which is held fixed) and not on $m$. 
\end{enumerate}
\begin{lem} \label{lemma: qf_cardinality_bounds_mom2} For any $\pi \in \part{1}{[2k+2]}$ we have,
\begin{align*}
    |\pi| & = \frac{2k+6+|\singleblks{\pi}| }{2} \implies |\cset{\pi}| \leq m^{\frac{2k+6+|\singleblks{\pi}| }{2}}. 
\end{align*}
For any $\pi \in \part{2}{[2k+2]}$, we have,
\begin{align*}
    |\pi| & \leq \frac{2k+5+|\singleblks{\pi}| }{2} \implies |\cset{\pi}| \leq m^{\frac{2k+5+|\singleblks{\pi}| }{2}}. 
\end{align*}
\end{lem}
\begin{proof}
Consider any $\pi \in \part{0}{[2k+2]}$.  Recall that the disjoint blocks of $|\pi|$ were given by:
\begin{align*}
        \pi = \fblknum{1}{\pi} \sqcup \lblknum{1}{\pi} \sqcup \fblknum{2}{\pi} \sqcup \lblknum{2}{\pi} \sqcup \left( \bigsqcup_{i \in \singleblks{\pi}} \{i\} \right) \sqcup \left( \bigsqcup_{t=1}^{|\pi| - |\singleblks{\pi}| - 4} \blocks_i\right).
    \end{align*}

Hence,
\begin{align*}
    2k+2 & = |\fblknum{1}{\pi}|+|\fblknum{2}{\pi}| + |\lblknum{1}{\pi}| + |\lblknum{2}{\pi}| + |\singleblks{\pi}| + \sum_{t=1}^{|\pi| - |\singleblks{\pi}| - 4} | \blocks_i|.
\end{align*}
Note that:
\begin{subequations}
\label{eq: qf_firstmom_blocksizeUB_observe_mom2}
\begin{align}
    |\fblknum{1}{\pi}| \geq 1 & \qquad \text{ (Since $1 \in \fblknum{1}{\pi}$)} \\
    |\fblknum{2}{\pi}| \geq 1 & \qquad \text{ (Since $k+2 \in \fblknum{2}{\pi}$)} \\
    |\lblknum{1}{\pi}| \geq 1 & \qquad \text{ (Since $k+1 \in \lblknum{1}{\pi}$)} \\
    |\lblknum{2}{\pi}| \geq 1 & \qquad \text{ (Since $2k+2 \in \lblknum{1}{\pi}$)} \\
    |\blocks_i| \geq 2 & \qquad \text{ (Since $\blocks_i$ are not singletons)}.
\end{align}\end{subequations}
Hence,
\begin{align*}
    2k+2 & \geq 4 +  2 |\pi| - |\singleblks{\pi}| - 8,
\end{align*}
which implies,
\begin{align}
     |\pi| &\leq  \frac{2k+6+|\singleblks{\pi}| }{2} \label{eq: qf_firstmom_blocksizeUB_mom2}, 
\end{align}
and hence,
\begin{align*}
    |\cset{\pi}| & \leq m^{|\pi|} \leq m^{\frac{2k+6+|\singleblks{\pi}| }{2}}.
\end{align*}
Finally observe that:
\begin{enumerate}
    \item For any $\pi \in \part{2}{[2k+2]}$ each of the inequalities in \eqref{eq: qf_firstmom_blocksizeUB_observe_mom2} are exactly tight by the definition of $\part{1}{[k+1]}$ in \eqref{eq: qf_firstmom_goodpartitions_mom2}, and hence,
    \begin{align*}
        |\pi| & = \frac{2k+6+|\singleblks{\pi}| }{2}.
    \end{align*}
    \item For any $\pi \in \part{2}{[2k+2]}$, one of the inequalities in \eqref{eq: qf_firstmom_blocksizeUB_observe_mom2} must be strict (see \eqref{eq: qf_firstmom_goodpartitions_mom2}). Hence, when $\pi \in \part{2}{[k+1]}$ we have the improved bound:
\begin{align*}
    |\pi| & \leq \frac{2k+5+|\singleblks{\pi}| }{2}.
\end{align*}
\end{enumerate}
This proves the claims of the lemma. 
\end{proof}
We will now show that $\mathsf{I}, \mathsf{II}, \mathsf{III} \rightarrow 0$.
\begin{lem} We have,
\begin{align*}
    \mathsf{I} \rightarrow 0, \; \mathsf{II} \rightarrow 0, \; \mathsf{III} \rightarrow 0 \;\text{ as $m \rightarrow \infty$},
\end{align*}
and hence,
\begin{align*}
    &\lim_{m \rightarrow \infty} \frac{\E (\bm z^\UT \altprod(\bm \Psi, \bm Z) \bm z)^2}{m^2}   = \\&\hspace{1cm} \lim_{m \rightarrow \infty} \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{a \in \cset{\pi}} \sum_{\bm w \in \weightedGnum{\pi}{2}} {\Coeff}(\bm w, \pi) \cdot \E\left[\matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right],
\end{align*}
provided the latter limit exists. 
\end{lem}
\begin{proof}
First note that for any $\bm w \in \weightedGnum{\pi}{1}$, we have,
\begin{align*}
    \|\bm w\| = \frac{1}{2} \sum_{i=1}^{2k+2} \degree_i(\bm w) = \frac{1+1 +1+1+ 2 |\singleblks{\pi}|}{2} = 2+ |\singleblks{\pi}| \; \text{ (See Lemma \ref{lemma: qf_mehler_conclusion_mom2})}.
\end{align*}
Furthermore recalling the definition of $\dlgraph$, $\|\dlgraph\| = 2k$.
Now we apply Lemma \ref{lemma: matrix_moment_ub} to obtain:
\begin{align*}
    |\E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \Indicator{\mathcal{E}^c} \right]|& \leq \sqrt{\E\left[   \matmom{\bm \Psi}{2\bm w + 2\dlgraph}{\pi}{\bm a} \right] } \sqrt{\P(\mathcal{E}^c)} \\
    &  \explain{}{\leq} \left( \frac{C_k \log^2(m)}{m} \right)^{\frac{|\singleblks{\pi}| + 2 + 2k}{2}} \cdot \sqrt{\P(\mathcal{E}^c)}, \\
    &\explain{(a)}{\leq} \left( \frac{C_k \log^2(m)}{m} \right)^{\frac{|\singleblks{\pi}| + 2 + 2k}{2}} \cdot \frac{C_k}{m}. \\
    \E|\matmom{\bm \Psi}{\dlgraph}{\pi}{\bm a}| &  \leq  \left( \frac{C_k \log^2(m)}{m} \right)^{k},\\
    \E\left[|\matmom{\bm \Psi}{\bm w + \bm{\ell}_{k+1}}{\pi}{\bm a}| \right] & \explain{}{\leq}  \left( \frac{C_k \log^2(m)}{m} \right)^{\frac{|\singleblks{\pi}| + 2 + 2k}{2}}
\end{align*}
In the step marked (a) we used Lemma \ref{lemma: trace_good_event}.
Further recall that by Lemma \ref{lemma: qf_mehler_conclusion} we have,
\begin{align*}
    |\epsilon(\bm \Psi, \bm a)| & \leq C(\altprod) \cdot \left( \frac{\log^3(m)}{m \kappa^2} \right)^{\frac{3 + |\singleblks{\pi}|}{2}}.
\end{align*}
Using these estimates, we obtain,
\begin{align*}
    |\mathsf{I}| & \leq  \frac{C(\altprod) \cdot }{m^2}  \cdot \sum_{\substack{\pi: \part{0}{[2k+2]}} }|\cset{\pi}| \cdot   \left( \frac{C_k \log^2(m)}{m}  \right)^{\frac{|\singleblks{\pi}| + 2 + 2k}{2}} \cdot\frac{C_k}{m}  \\& \leq   \frac{C(\altprod) \cdot }{m^2}  \cdot \sum_{\substack{\pi: \part{0}{[2k+2]}} }m^{\frac{2k+6+|\singleblks{\pi}|}{2}} \cdot   \left( \frac{C_k \log^2(m)}{m} \right)^{\frac{|\singleblks{\pi}| + 2 + 2k}{2}} \cdot \frac{C_k}{m}\\
    & = O \left( \frac{\polylog(m)}{m} \right)\\
    |\mathsf{II}| & \leq \frac{C(\altprod)}{m^2} \cdot \left( \frac{C_k \log^2(m)}{m} \right)^{k} \cdot  \sum_{\substack{\pi: \part{0}{[2k+2]}}}  |\cset{\pi}|  \cdot \left( \frac{\log^3(m)}{m \kappa^2} \right)^{\frac{3 + |\singleblks{\pi}|}{2}} \\&\leq \frac{C(\altprod)}{m^2} \cdot \left( \frac{C_k \log^2(m)}{m} \right)^{{k}} \cdot  \sum_{\substack{\pi: \part{0}{[2k+2]} } }  m^{\frac{2k+6+|\singleblks{\pi}|}{2}}  \cdot \left( \frac{\log^3(m)}{m \kappa^2} \right)^{\frac{3 + |\singleblks{\pi}|}{2}} \\
     & = O \left( \frac{\polylog(m)}{\sqrt{m}} \right)\\
    |\mathsf{III}| & \leq \frac{C(\altprod) \cdot }{m^2}  \cdot \sum_{\pi: \part{2}{[2k+2]}  }|\cset{\pi}| \cdot   \left( \frac{C_k \log^2(m)}{m} \right)^{\frac{|\singleblks{\pi}| + 1 + k}{2}} \\
    & \leq \frac{C(\altprod) \cdot }{m^2}  \cdot \sum_{\pi: \part{2}{[2k+2]}  } m^{\frac{2k+5+|\singleblks{\pi}|}{2}} \cdot   \left( \frac{C_k \log^2(m)}{m} \right)^{\frac{|\singleblks{\pi}| + 2 + 2k}{2}} \\
    &=O \left( \frac{\polylog(m)}{\sqrt{m}} \right).
\end{align*}
This concludes the proof of this lemma.
\end{proof}

Next, we consider the decomposition:
\begin{align*}
    & \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{a \in \cset{\pi}} \sum_{\bm w \in \weightedGnum{\pi}{2}} {\Coeff}(\bm w, \pi) \cdot \E\left[\matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right] = \\& \hspace{0cm} \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph  \in \weightedGnum{\pi}{DA}}} \sum_{a \in \labelling{CF}(\bm w + \dlgraph, \pi)}  {\Coeff}(\bm w, \pi) \cdot \E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right] + \mathsf{IV} + \mathsf{V},
\end{align*}
where,
\begin{align*}
    \mathsf{IV} &\explain{def}{=}  \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{a \in \cset{\pi}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph \notin \weightedGnum{\pi}{DA}}} {\Coeff}(\bm w, \pi) \cdot \E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right], \\
    \mathsf{V} &\explain{def}{=} \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph \in \weightedGnum{\pi}{DA}}} \sum_{a \in \cset{\pi} \backslash \labelling{CF}(\bm w + \dlgraph, \pi)}  {\Coeff}(\bm w, \pi) \cdot \E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right].
\end{align*}
\begin{lem}
We have, $\mathsf{IV} \rightarrow 0, \mathsf{V} \rightarrow 0$ as $m \rightarrow \infty$, and hence,
\begin{align*}
    &\lim_{m \rightarrow \infty} \frac{\E (\bm z^\UT \altprod \bm z)^2}{m^2}  =\\& \hspace{0cm} \lim_{m \rightarrow \infty}  \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph  \in \weightedGnum{\pi}{DA}}} \sum_{a \in \labelling{CF}(\bm w + \dlgraph, \pi)}  {\Coeff}(\bm w, \pi) \cdot \E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right],
\end{align*}
provided the latter limit exists. 
\end{lem}
\begin{proof}
We will prove this in two steps.
\begin{description}
\item [Step 1: $\mathsf{IV} \rightarrow 0$. ] We consider the two sensing models separately:
\begin{enumerate}
    \item Subsampled Hadamard Sensing: In this case, Proposition \ref{prop: clt_hadamard} tells us that if $\bm w + \dlgraph \not\in \weightedGnum{\pi}{DA}$, then, $$\E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right] = 0$$ and hence $\mathsf{IV} = 0$.
    \item Subsampled Haar Sensing: Observe that, since $\|\bm w\| + \|\dlgraph\|= 2 + |\singleblks{\pi}| + 2k$, we have,
    \begin{align*}
        \E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right] & = \frac{\E\left[   \matmom{\sqrt{m}\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right]}{m^{\frac{2 + |\singleblks{\pi}| + 2k}{2}}}.
    \end{align*}
    By Proposition \ref{prop: clt_random_ortho} we know that,
    \begin{align*}
        \left| \E\left[   \matmom{\sqrt{m}\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right] - \prod_{\substack{s,t \in [|\pi|] \\ s \leq t}} \E \left[ Z_{st}^{W_{st}(\bm w + \dlgraph, \pi)} \right] \right| & \leq \frac{K_1 \log^{K_2}(m)}{m^\tbd},
    \end{align*}
    $ \; \forall \; m \geq K_3$, where $K_1,K_2,K_3$ are universal constants depending only on $k$. Note that since $\bm w + \dlgraph \notin \weightedGnum{\pi}{DA}$, must have some $s \in [|\pi|]$ such that:
    \begin{align*}
        W_{ss}(\bm w + \dlgraph, \pi) \geq 1.
    \end{align*}
    Recall that, $\degree_i(\bm w) = 0$ for any $i \not\in \{1,k+1,k+2,2k+2\} \cup \singleblks{\pi}$ (since $\bm w \in \weightedGnum{\pi}{2}$) and furthermore, $|\pi(i)| = 1 \forall \; i \; \in \; \{1,k+1,k+2,2k+2\} \cup \singleblks{\pi}$ (since $\pi \in \part{1}{2k+2}$). Hence, we have $\bm w \in \weightedGnum{\pi}{DA}$ and in particular, $W_{ss}(\bm w, \pi) =0$. Consequently, we must have $W_{ss}(\dlgraph, \pi) \geq 1$. Recall the definition of $\dlgraph$, since $W_{ss}(\bm{\ell}_{k+1}, \pi) \geq 1$ we must have that for some $i \in [2k+2]$, we have, $\pi(i) = \pi(i+1) = \blocks_s$. However, since $\pi \in \part{1}{2k+2}$, $|\blocks_s| \leq 2$, and hence $\blocks_s = \{i,i+1\}$. This means that $W_{ss}(\dlgraph,\pi) = 1 =W_{ss}(\bm w + \dlgraph, \pi)$. Consequently since $\E Z_{ss} = 0$, we have,
    \begin{align*}
        \prod_{\substack{s,t \in [|\pi|] \\ s \leq t}} \E \left[ Z_{st}^{W_{st}(\bm w + \dlgraph, \pi)} \right] = 0,
    \end{align*}
    or,
    \begin{align*}
        \left|\E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right]\right| & = \frac{\polylog(m)}{m^{\frac{2 + |\singleblks{\pi}| + 2k}{2}+\tbd}}.
    \end{align*}Recalling Lemma \ref{lemma: qf_cardinality_bounds_mom2},
    \begin{align*}
        |\cset{\pi}| & \leq m^{|\pi|} \leq m^{\frac{2k+6+|\singleblks{\pi}| }{2}},
    \end{align*}
    we obtain,
    \begin{align*}
        |\mathsf{IV}| & \leq \frac{C(\altprod)}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} |\cset{\pi}|  \cdot  \frac{\polylog(m)}{m^{\frac{2 + |\singleblks{\pi}| + 2k}{2}+\tbd}} = O\left( \frac{\polylog(m)}{m^\tbd}\right) \rightarrow 0.
    \end{align*}
\end{enumerate}
\item [Step 2: $\mathsf{V} \rightarrow 0$. ]  Using Lemma \ref{lemma: cf_size_bound}, we know that $$|\cset{\pi} \backslash \labelling{CF}(\bm w+\dlgraph, \pi)| \leq O( m^{|\pi|-1})$$
In Lemma \ref{lemma: qf_cardinality_bounds_mom2}, we showed that for any $\pi \in \part{1}{[k+1]}$, 
\begin{align*}
    |\pi| & = \frac{2k+6+|\singleblks{\pi}| }{2}.
\end{align*}
Hence,
\begin{align*}
    |\cset{\pi} \backslash \labelling{CF}(\bm w+\dlgraph, \pi)| &\leq O( m^{\frac{2k+4+|\singleblks{\pi}| }{2}}).
\end{align*}
We already know from Lemma \ref{lemma: matrix_moment_ub} that,
\begin{align*}
    | \E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right]| & \leq \left( \frac{C_k \log^2(m)}{m} \right)^{\frac{\|\bm w\| + \|\dlgraph\|}{2}} \explain{}{\leq} \left( \frac{C_k \log^2(m)}{m} \right)^{\frac{|\singleblks{\pi}| + 2 + 2k}{2}},
\end{align*}
This gives us:
\begin{align*}
    |\mathsf{V}| & \leq \frac{C}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph \in \weightedGnum{\pi}{DA}}}  |\cset{\pi} \backslash \labelling{CF}(\bm w+\dlgraph, \pi)|  \left( \frac{C_k \log^2(m)}{m} \right)^{\frac{|\singleblks{\pi}| + 2 + 2k}{2}} \\
    & = O \left( \frac{\polylog(m)}{m} \right)
\end{align*}
which goes to zero as claimed.
\end{description}
This concludes the proof of the lemma.
\end{proof}
So far we have shown that:
\begin{align*}
    &\lim_{m \rightarrow \infty} \frac{\E (\bm z^\UT \altprod \bm z)^2}{m^2}   = \\& \lim_{m \rightarrow \infty}  \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph  \in \weightedGnum{\pi}{DA}}} \sum_{a \in \labelling{CF}(\bm w + \dlgraph, \pi)}  {\Coeff}(\bm w, \pi) \cdot \E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right].
\end{align*}
provided the latter limit exists. In the following lemma we explicitly calculate the limit on the RHS and hence show that it exists and is same for the subsampled Haar and subsampled Hadamard sensing models. 
\begin{lem}\label{lemma: mom2_complex_formula} For both the subsampled Haar sensing and Hadamard sensing model, we have,
\begin{align*}
    \lim_{m \rightarrow \infty} \frac{\E (\bm z^\UT \altprod \bm z)^2}{m^2}  & = \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph \in \weightedGnum{\pi}{DA}}}   {\Coeff}(\bm w, \pi) \cdot\limmom{\bm w+\dlgraph}{\pi},
\end{align*}
where,
\begin{align*}
    \limmom{\bm w+\dlgraph}{\pi} &\explain{def}{=}  \prod_{\substack{s,t \in [|\pi|] \\ s < t}} \E \left[ Z^{W_{st}(\bm w + \dlgraph, \pi)} \right], \; Z \sim \gauss{0}{\kappa(1-\kappa)}.
\end{align*}
\end{lem}
\begin{proof}
By Propositions \ref{prop: clt_hadamard} (for the subsampled Hadamard model) and \ref{prop: clt_random_ortho} (for the subsampled  Haar model) we know that, if $\bm w + \dlgraph \in \weightedGnum{\pi}{DA}, \; \bm a  \in \labelling{CF}(\bm w+\dlgraph, \pi)$, we have,
\begin{align*}
    \matmom{\sqrt{m}\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} & = \limmom{\bm w+\dlgraph}{\pi} + \epsilon(\bm w, \pi, \bm a),
\end{align*}
where
\begin{align*}
     |\epsilon(\bm w, \pi, \bm a)| & \leq \frac{K_1 \log^{K_2}(m)}{m^\tbd}, \; \forall \; m \geq K_3,
\end{align*}
for some constants $K_1,K_2,K_3$ depending only on $k$. Hence, we can consider the decomposition:
\begin{align*}
   \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph  \in \weightedGnum{\pi}{DA}}} \sum_{a \in \labelling{CF}(\bm w + \dlgraph, \pi)}  {\Coeff}(\bm w, \pi) \cdot & \E\left[   \matmom{\bm \Psi}{\bm w + \dlgraph}{\pi}{\bm a} \right] \\& = \mathsf{VI} + \mathsf{VII},
\end{align*}
where,
\begin{align*}
    \mathsf{VI} & \explain{def}{=} \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph  \in \weightedGnum{\pi}{DA}}} \sum_{a \in \labelling{CF}(\bm w + \dlgraph, \pi)}  {\Coeff}(\bm w, \pi) \cdot  \frac{\limmom{\bm w+\dlgraph}{\pi}}{m^{\frac{2 + \singleblks{\pi} + 2k}{2}}}, \\
    \mathsf{VII} & \explain{def}{=} \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph  \in \weightedGnum{\pi}{DA}}} \sum_{a \in \labelling{CF}(\bm w + \dlgraph, \pi)}  {\Coeff}(\bm w, \pi) \cdot   \frac{\epsilon(\bm w, \pi, \bm a)}{m^{\frac{2 + \singleblks{\pi} + 2k}{2}}}
\end{align*}
We can upper bound $|\mathsf{VII}|$ as follows:
\begin{align*}
    |\labelling{CF}(\bm w+\dlgraph, \pi)| & \leq |\cset{\pi}| \explain{}{\leq} m^{\frac{2k+6+|\singleblks{\pi}|}{2}}, \\
|\mathsf{VII}| & \leq \frac{C(\altprod)}{m^2} \cdot C_k \cdot |\labelling{CF}(\bm w+\dlgraph, \pi)| \cdot \frac{1}{m^{\frac{2 + |\singleblks{\pi}| + 2k}{2}}} \cdot  \frac{K_1 \log^{K_2}(m)}{m^\tbd} \\&= O\left( \frac{\polylog(m)}{m^\tbd} \right) \rightarrow 0.
\end{align*}
We can compute:
\begin{align*}
    &\lim_{m \rightarrow \infty} (\mathsf{VI})  = \lim_{m \rightarrow \infty} \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph  \in \weightedGnum{\pi}{DA}}} \sum_{a \in \labelling{CF}(\bm w + \dlgraph, \pi)}  {\Coeff}(\bm w, \pi) \cdot  \frac{\limmom{\bm w+\dlgraph}{\pi}}{m^{\frac{2 + \singleblks{\pi} + 2k}{2}}} \\
    & = \lim_{m \rightarrow \infty} \frac{1}{m^2} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph  \in \weightedGnum{\pi}{DA}}}   {\Coeff}(\bm w, \pi) \cdot  \frac{\limmom{\bm w+\dlgraph}{\pi}}{m^{\frac{2 + \singleblks{\pi} + 2k}{2}}} \cdot |\labelling{CF}(\bm w+\dlgraph, \pi)| \\
    & =  \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph  \in \weightedGnum{\pi}{DA}}}  {\Coeff}(\bm w, \pi) \cdot \limmom{\bm w+\dlgraph}{\pi} \cdot \frac{m^{|\pi|}}{m^{\frac{6 + \singleblks{\pi} + 2k}{2}}} \cdot \frac{|\labelling{CF}(\bm w+\dlgraph, \pi)|}{m^{|\pi|}} \\
    & \explain{(a)}{=} \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph  \in \weightedGnum{\pi}{DA}}}  {\Coeff}(\bm w, \pi) \cdot \limmom{\bm w+\dlgraph}{\pi} \cdot  \frac{|\labelling{CF}(\bm w+\dlgraph, \pi)|}{m^{|\pi|}} \\
    & \explain{(b)}{=}  \sum_{\pi \in \part{1}{[2k+2]}} \sum_{\substack{\bm w \in \weightedGnum{\pi}{2}\\ \bm w + \dlgraph  \in \weightedGnum{\pi}{DA}}}  {\Coeff}(\bm w, \pi) \cdot \limmom{\bm w+\dlgraph}{\pi} .
\end{align*}
In the step marked (a) we used the fact that $|\pi| = (6 + |\singleblks{\pi}| +2k)/2$ for any $\pi \in \part{1}{[2k+2]}$ (Lemma \ref{lemma: qf_cardinality_bounds_mom2}) and in step (b) we used Lemma \ref{lemma: cf_size_bound} ($|\labelling{CF}(\bm w+\dlgraph, \pi)|/m^{|\pi|} \rightarrow 1$).
This proves the claim of the lemma and Proposition \ref{prop: qf_univ_mom2}.
\end{proof}
We can actually significantly simply the combinatorial sum obtained in Lemma \ref{lemma: mom2_complex_formula} which we do so in the following lemma.

\begin{lem}For both the subsampled Haar sensing and Hadamard sensing models, we have,
\begin{align*}
     \lim_{m \rightarrow \infty} \frac{\E (\bm z^\UT \altprod \bm z)^2}{m^2}& =  (1-\kappa)^{2k} \cdot \prod_{i=1}^{k-1} \hat{q}^2_i(2).
\end{align*}
In particular, Proposition \ref{prop: qf_univ_mom2} holds. 
\end{lem}
\begin{proof}
We claim that the only partition with a non-zero contribution is:
\begin{align*}
    \pi & = \bigsqcup_{i=1}^{2k+2}\{i\}.
\end{align*}
In order to see this suppose $\pi$ is not entirely composed of singleton blocks. Define:
\begin{align*}
    i_\star & \explain{def}{=}\min  \{i \in [2k+2]: |\pi(i)| > 1  \}.
\end{align*}
Note $i_\star > 1$ since we know that $|\pi(1)| = |\fblknum{1}{\pi}| = 1$ for any $\pi \in \part{1}{2k+2}$.
Since $\pi \in \part{1}{[2k+2]}$ we must have $|\pi(i_\star)| = 2$, hence denote:
\begin{align*}
    \pi(i_\star)= \{i_\star, j_\star\}.
\end{align*}
for some $j_\star > i_\star+1$ ($i_\star \leq j_\star$ since it is the first index which is not in a singleton block, and $j_\star \neq i_\star + 1$ since otherwise $\bm w + \dlgraph$ will not be disassortative. Similarly we know that $i_\star,j_\star \neq k+1,k+2,2k+2$ because $|\pi(k+1)| = |\pi(k+2)| = |\pi(2k+2)| = 1$ since $\pi \in \part{1}{[2k+2]}$.
Let us label the first few blocks of $\pi$ as:
\begin{align*}
    \blocks_1 = \{1\}, \; \blocks_2 = \{2\}, \dots \blocks_{i_\star - 1} = \{i_\star - 1\}, \; \blocks_{i_\star} = \{i_\star, j_\star\}.
\end{align*}
Next we compute:
\begin{align*}
    W_{i_\star-1,i_\star}(\bm w + \dlgraph, \pi) & = W_{i_\star-1,i_\star}(\dlgraph, \pi) + W_{i_\star-1,i_\star}(\bm w , \pi) \\
    & \explain{(a)}{=} W_{i_\star-1,i_\star}(\dlgraph, \pi) \\
    & \explain{(b)}{=} \mathbf{1}_{i_{\star} - 1 \in \blocks_{i_\star-1}}  + \mathbf{1}_{i_{\star} + 1 \in \blocks_{i_\star-1}} + \mathbf{1}_{j_{\star} - 1 \in \blocks_{i_\star-1}}  + \mathbf{1}_{j_{\star} + 1 \in \blocks_{i_\star-1}} \\
    & \explain{(c)}{=} \mathbf{1}_{i_{\star} - 1 = {i_\star-1}}  + \mathbf{1}_{i_{\star} + 1 ={i_\star-1}} + \mathbf{1}_{j_{\star} - 1 ={i_\star-1}}  + \mathbf{1}_{j_{\star} + 1 = {i_\star-1}} \\
    & \explain{(d)}{=} 1.
\end{align*}
In the step marked (a), we used the fact that since $\bm w \in \weightedGnum{\pi}{2}$ and $|\pi(i_\star)| = |\pi(j_\star)| = 2$, we must have $d_{i_\star}(\bm w) = d_{j_\star}(\bm w) = 0$ and $W_{i_\star-1,i_\star}(\bm w, \pi) = 0$. In the step marked (b) we used the definition of $\dlgraph$. In the step marked (c) we used the fact that $\blocks_{i_\star-1} = \{i_{\star-1}\}$. In the step marked (d) we used the fact that $j_\star > i_\star + 1$.

Hence we have shown that for any $\pi \neq \sqcup_{i=1}^{2k+2} \{i\}$, we have 
\begin{align*}
    \mu(\bm w, \pi) = 0 \; \forall \; \bm w \text{ such that}  \; \bm w \in \weightedGnum{\pi}{2}, \; \bm w + \dlgraph \in \weightedGnum{\pi}{DA}.
\end{align*}
Next, let $\pi = \sqcup_{i=1}^{2k+2} \{i\}$. We observe for any $\bm w$ such that $\bm w \in \weightedGnum{\pi}{2}, \; \bm w + \dlgraph \in \weightedGnum{\pi}{DA}$, we have,
\begin{align*}
    \limmom{\bm w+ \dlgraph}{\pi} &\explain{}{=}  \prod_{\substack{s,t \in [|\pi|] \\ s < t}} \E \left[ Z^{W_{st}(\bm w + \dlgraph, \pi)} \right], \; Z \sim \gauss{0}{\kappa(1-\kappa)} \\
    & = \prod_{\substack{i,j \in [2k+2] \\ i < j}} \E \left[ Z^{w_{ij} + ({\ell}_{k+1})_{ij}, \pi)} \right], \; Z \sim \gauss{0}{\kappa(1-\kappa)}
\end{align*}
Note that since $\E Z = 0$, for $\limmom{\bm w + \dlgraph}{\pi} \neq 0$ we must have:
\begin{align*}
    w_{ij} \geq (\dlgraph)_{ij}, \; \forall \; i,j \; \in \; [2k+2].
\end{align*}
However since $\bm w \in \weightedGnum{\pi}{2}$ we have,
\begin{align*}
    \degree_1(\bm w) &= \degree_{k+1}(\bm w)=\degree_{k+2}(\bm w) = \degree_{2k+2}(\bm w) = 1, \\ \degree_i(\bm w) &= 2 \; \forall \; i \; \in \; [2k+2]\backslash\{1,k+1,k+2,2k+2\},
\end{align*}
hence $\bm w = \dlgraph$. Hence, recalling the formula for $\coeff(\bm w, \pi)$ from Lemma \ref{lemma: qf_mehler_conclusion} we obtain:
\begin{align*}
     \lim_{m \rightarrow \infty} \frac{\E (\bm z^\UT \altprod \bm z)^2}{m^2}& =  (1-\kappa)^{2k} \cdot \prod_{i=1}^{k-1} \hat{q}^2_i(2).
\end{align*}
This proves the statement of the lemma and also Proposition \ref{prop: qf_univ_mom1} (see Remark \ref{remark: all_types_qf_mom1} regarding how the analysis extends to other types).
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% PROOF-CLT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proofs from Section \ref{section: clt}}
\label{appendix: clt}

\subsection{Proof of Lemma \ref{lemma: matrix_moment_ub}} \label{proof: matrix_moment}

\begin{proof}[Proof of Lemma \ref{lemma: matrix_moment_ub}]
Recall that,
\begin{align*}
    \E|\matmom{\bm \Psi}{\bm w}{\pi}{\bm a}| & = \E\prod_{\substack{i,j \in [k] \\ i < j}} |\Psi_{a_i,a_j}^{w_{ij}}| \\
    & \explain{(a)}{\leq} \sum_{\substack{i,j \in [k] \\ i < j}} \frac{w_{ij}}{\|\bm w\|} \E |\Psi_{a_i,a_j}^{\|\bm w\|_1}| \\
    & \leq \max_{i,j \in [m] } \E |\Psi_{ij}|^{\|\bm w\|},
\end{align*}
where step $(a)$ follows from the AM-GM inequality. We now consider the subsampled Haar and Hadamard cases separately.
\begin{description}
\item [Hadamard Case: ] By Lemma \ref{concentration}, $\Psi_{ij}$ is subgaussian with with variance proxy bounded by $C/m$ for some universal constant $C$. Hence, 
\begin{align*}
     \E|\matmom{\bm \Psi}{\bm w}{\pi}{\bm a}| &  \leq  \left( \frac{C\|\bm w\|}{m} \right)^{\frac{\|\bm w\|}{2}}.
\end{align*}
\item [Haar Case: ] By Lemma \ref{concentration}, conditional on $\bm O$, $\Psi_{ij}$ is subgaussian with variance proxy $C m \|\bm o_i\|_\infty^2 \|\bm o_j\|_\infty^2$. Hence,
\begin{align*}
    \E|\matmom{\bm \Psi}{\bm w}{\pi}{\bm a}| & \leq \max_{i,j \in [m] } \E |\Psi_{ij}|^{\|\bm w\|}\\
    & = \max_{i,j \in [m] } \E [\E[|\Psi_{ij}|^{\|\bm w\|} | \bm O]] \\
    & \leq \max_{i,j \in [m]} (C\|\bm w\| m)^{\frac{\|\bm w\|}{2}} \E\left[ \|\bm o_i\|_\infty^{\|\bm w\|} \|\bm o_j\|_\infty^{\|\bm w\|}  \right] \\
    & \leq \max_{i,j \in [m]} (C\|\bm w\| m)^{\frac{\|\bm w\|}{2}} \left( \E \|\bm o_i\|_\infty^{2 \|\bm w\|} + \E \|\bm o_j\|_\infty^{2\|\bm w\|} \right).
\end{align*}
Note that $\bm o_i \explain{d}{=} \bm o_j \explain{d}{=} \bm u \sim \unif{\mathbb{S}_{m-1}}$. Applying Fact \ref{fact: infty_norm_uniform_unit} gives us,
\begin{align*}
    \E |\matmom{\bm \Psi}{\bm w}{\pi}{\bm a}|  & \leq \left( \sqrt{\frac{C \|\bm w\| \log^2(m)}{m}} \right)^{\|\bm w\|}.
\end{align*}
\end{description}
\end{proof}

\subsection{Proofs of Propositions \ref{prop: clt_random_ortho} and \ref{prop: clt_hadamard}}
\label{proof: clt_props}
This section is dedicated to the proof of Propositions \ref{prop: clt_random_ortho} and \ref{prop: clt_hadamard}. We consider the following general setup. Let $\bm v_1, \bm v_2 \cdots, \bm v_m $ be fixed vectors in $\R^d$ for a fixed $d \in \N$. Define the statistic:
\begin{align*}
    \bm T & = \sqrt{m}\sum_{i=1}^m \overline{B}_{ii} \bm v_i,
\end{align*}
where $\barB$ denotes a diagonal matrix whose $n$ diagonal entries are set to $1-\kappa$ uniformly at random and the remaining $m-n$ are set to $-\kappa$.

Analogously, we define the statistic:
\begin{align*}
    \hat{\bm T} & = \sqrt{m}\sum_{i=1}^m \hat{B}_{ii} \bm v_i,
\end{align*}
where,
\begin{align*}
    \hat{B}_{ii} & \explain{i.i.d.}{\sim} \begin{cases} 1- \kappa : & \text{with prob. } \kappa \\ -\kappa: & \text{with prob. } 1-\kappa \end{cases}.
\end{align*}
As in the proof of Lemma \ref{concentration} we define $\barB$ and $\hat{\bm B}$ in the same probability space as follows:
\begin{enumerate}
    \item We first sample $\barB$. Let $S = \{i \in [m]: \overline{B}_{ii} = 1-\kappa \}$
    \item Next sample $N \sim \bnomdistr{m}{\kappa}$.
    \item Sample a subset $\hat{S} \subset [m]$ with $|\hat{S}| = N$ as follows:
    \begin{itemize}
        \item If $N\leq n$, then set $\hat{S}$ to be a uniformly random subset of $S$ of size $N$.
        \item If $N>n$ first sample a uniformly random subset $A$ of $S^c$ of size $N-n$ and set $\hat{S} = S \cup A $
    \end{itemize}
    \item Set $\hat{\bm B}$ as follows:
    \begin{align*}
        \hat{B}_{ii} & = \begin{cases} -\kappa &: i \not\in \hat{S} \\ 1-\kappa &: i \in \hat{S}. \end{cases}.
    \end{align*}
\end{enumerate}
We stack the vectors $\bm v_{1:m}$ along the rows of a matrix $\bm V \in \R^{m\times d}$ and refer to the columns of $\bm V$ as $\bm V_1, \bm V_2 \cdots \bm V_d$:
\begin{align*}
    \bm V = [\bm V_1, \bm V_2 \cdots \bm V_d] = \begin{bmatrix} \bm v_1^\UT \\ \bm v_2^\UT \\ \vdots \\ \bm v_m^\UT \end{bmatrix}.
\end{align*}

Lastly we introduce the matrix $\hat{\bm \Sigma} \in \R^{d \times d}$:
\begin{align*}
    \hat{\bm \Sigma} &\explain{def}{=} \E[\hat{\bm T} \hat{\bm T}^\UT | \bm V] = m \kappa(1-\kappa) \bm V^\UT \bm V.
\end{align*}
These definitions are intended to capture the matrix moments $\matmom{\bm \Psi}{\bm w}{\pi}{\bm a}$ as follows:  Consider any $k \in \N, \pi \in \part{}{[k]}, \bm w \in \weightedG{k}$ and any $\bm a \in \cset{\pi}$. Let the disjoint blocks of $\pi$ be given by $\pi = \blocks_1 \sqcup \blocks_2 \cdots \sqcup \blocks_{|\pi|}$.

In order to capture $\matmom{\bm \Psi}{\bm w}{\pi}{\bm a}$ in the subsampled Hadamard case $\bm \Psi = \bm H \barB \bm H^\UT$ and the subsampled Haar case $\bm \Psi = \bm O \barB \bm O^\UT$ we will set $\bm V_{1:d}$ as follows:
\begin{enumerate}
    \item In the subsampled Haar case, we set:
    \begin{align*}
        \{\bm V_1, \bm V_2, \cdots \bm V_d \} = \{ (\bm o_{a_{\blocks_s}} \odot \bm o_{a_{\blocks_t}}) - \delta(s,t) \hat{\bm e}: s,t \in [|\pi|], \; s \leq t, \; W_{st}(\bm w, \pi) > 0 \},
    \end{align*}
    where,
    \begin{align*}
        \bm e^\UT = \left( \frac{1}{{m}}, \frac{1}{{m}} \cdots \frac{1}{{m}} \right), \; \delta(s,t) = \begin{cases} 1 : & s = t \\ 0 : & s \neq t \end{cases}.
    \end{align*}
    If for some $i \in [d]$ and some $s,t \in [|\pi|]$ we have $\bm V_i =  \bm o_{a_{\blocks_s}} \odot \bm o_{a_{\blocks_t}} - \delta(s,t) \hat{\bm e}$,
    we will abuse notation and often refer to $\bm V_i$ as $\bm V_{st}$. Likewise the corresponding entries of $\bm T, \hat{\bm T}$, $T_i, \hat{T}_i$ will be referred to as $T_{st}, \hat{T}_{st}$.
    \item In the subsampled Hadamard case, we set:
    \begin{align*}
        \{\bm V_1, \bm V_2, \cdots \bm V_d \} = \{  \bm h_{a_{\blocks_s}} \odot \bm h_{a_{\blocks_t}} - \delta(s,t) \hat{\bm e}: s,t \in [|\pi|], \; s \leq t, \; W_{st}(\bm w, \pi) > 0 \}.
    \end{align*}
    If for some $i \in [d]$ and some $s,t \in [|\pi|]$ we have $\bm V_i =  \bm h_{a_{\blocks_s}} \odot \bm h_{a_{\blocks_t}}-\delta(s,t) \hat{\bm e}$, 
    we will abuse notation and often refer to $\bm V_i$ as $\bm V_{st}$. Likewise the corresponding entries of $\bm T, \hat{\bm T}$:  $T_i, \hat{T}_i$ will be referred to as $T_{st}, \hat{T}_{st}$.
\end{enumerate}
With the above conventions and the observation that $\sum_{i=1}^m \overline{B}_{ii} = 0$ we have:
\begin{align*}
    \matmom{ \sqrt{m}\bm \Psi}{\bm w}{\pi}{\bm a} & = \prod_{\substack{s,t \in [|\pi|]\\ s \leq t \\ W_{st} (\bm w, \pi) > 0}} T_{st}^{W_{st}(\bm w, \pi)}.
\end{align*}

The remainder of this section is organized as follows:
\begin{enumerate}
    \item First, in Lemma \ref{lemma: asymptotic covariance} we show that $\hat{\bm \Sigma}$ converges to a fixed deterministic matrix $\bm \Sigma$ and bound the rate of convergence in terms of $\E \|\hat{\bm \Sigma} - \bm \Sigma \|_\fr^2$.
    \item In Lemma \ref{lemma: coupling exact form} we upper bound $\E \|\hat{\bm T} - \bm T\|_2^2$. Consequently a Gaussian approximation result for $\hat{\bm T}$ implies a Gaussian approximation result for $\bm T$.
    \item In Lemma \ref{lemma: berry_eseen}, we use a standard Berry-Esseen bound of \citet{bhattacharya1975errors} to derive a Gaussian approximation result for $\hat{\bm T}$ since it is a weighted sum of i.i.d. centered random variables.
    \item Finally we conclude by using the above lemmas to provide a proof for Propositions \ref{prop: clt_hadamard} and \ref{prop: clt_random_ortho}.
\end{enumerate}

\begin{lem}  \label{lemma: asymptotic covariance}
\begin{enumerate}
    \item For the Hadamard case suppose $\bm w$ is disassortative with respect to $\pi$ and $\bm a$ is a conflict free labelling of $(\bm w, \pi)$. Then,
    \begin{align*}
        \hat{\bm \Sigma} = \kappa(1-\kappa)\bm I_d.
    \end{align*}
    \item For the Haar case there exists a universal constant $C < \infty$ such that for any partition $\pi \in \part{}{[k]}$, any weight matrix $\bm w \in \weightedG{k}$ and any labelling $\bm a \in \cset{\pi}$ we have,
    \begin{align*}
        \E \|\hat{\bm \Sigma} - \bm \Sigma \|_\fr^2 & \leq  \frac{C\cdot k^4 \cdot (\kappa^2 (1-\kappa)^2)}{m}.
    \end{align*}
    where the matrix $\bm \Sigma$ is a diagonal matrix whose diagonal entries are given by:
    \begin{align*}
        \Sigma_{st,st} & = \begin{cases} \kappa(1-\kappa) : & s\neq t \\ 2 \kappa(1-\kappa) : & s = t \end{cases}.
    \end{align*}
\end{enumerate}
\end{lem}

\begin{proof} Recall that,
\begin{align*}
    \hat{\bm \Sigma} & = m \kappa(1-\kappa) \bm V^\UT \bm V.
\end{align*}

We consider the Hadamard and the Haar case separately. 
\begin{description}
\item [Hadamard Case: ] Consider two pairs $(s,t)$ and $(s^\prime,t^\prime)$ such that:
\begin{align*}
    s \leq t, \; W_{st}(\bm w, \pi) > 0, \; s, t \; \in \;  [|\pi|].
\end{align*}
and the analogous assumptions on the pair $(s^\prime,t^\prime)$.
Then the entry $\hat{\Sigma}_{st,s^\prime t^\prime}$ is given by:
\begin{align*}
    \hat{\Sigma}_{st,s^\prime t^\prime} & = m \kappa(1-\kappa) \ip{\bm V_{st}}{\bm V_{s^\prime t^\prime}} \\
    & = m \kappa(1-\kappa) \ip{\bm h_{a_{\blocks_s}}  \odot \bm  h_{a_{\blocks_t}} - \delta(s,t) \hat{\bm e}}{\bm h_{a_{\blocks_s^\prime}}  \odot \bm  h_{a_{\blocks_t^\prime}}-\delta(s^\prime,t^\prime) \hat{\bm e}} \\
    & \explain{(a)}{=} \kappa(1-\kappa)\ip{\bm h_{a_{\blocks_s} \oplus a_{\blocks_t}}  - \sqrt{m}\delta(s,t) \hat{\bm e}}{\bm h_{a_{\blocks_s^\prime}\oplus a_{\blocks_t^\prime}}-\sqrt{m}\delta(s^\prime,t^\prime) \hat{\bm e}} \\
    & \explain{(b)}{=}\kappa(1-\kappa) \ip{\bm h_{a_{\blocks_s} \oplus a_{\blocks_t}}}{\bm h_{a_{\blocks_s^\prime}\oplus a_{\blocks_t^\prime}}} \\
    &\explain{(c)}{=} \kappa(1-\kappa)\delta(s,s^\prime) \delta(t,t^\prime).
\end{align*}
In the step marked (a) we appealed to Lemma \ref{lemma: hadamard_key_property}. In the step marked (b), we noted that $\hat{\bm e} = \bm h_1/\sqrt{m}$ and $\hat{\bm e} \perp \bm h_{a_{\blocks_s} \oplus a_{\blocks_t}}$ unless $s = t$ which is ruled out by the fact that $\bm w$ is disassortative with respect to $\pi$ i.e. $W_{ss}(\bm w,\pi) = 0$. In the step marked (c) we used the fact that $\bm a$ is a conflict free labelling. Consequently, we have shown that $\hat{\bm \Sigma} = \kappa(1-\kappa)\bm I_d$.
\item [Haar case: ] By the bias-variance decomposition:
\begin{align*}
    \E \|\hat{\bm \Sigma} - \bm \Sigma \|_\fr^2 & = \E \|\hat{\bm \Sigma} - \E\hat{\bm \Sigma} \|_\fr^2 + \|\E\hat{\bm \Sigma} - \bm \Sigma \|_\fr^2.
\end{align*}
We will first compute $\E \hat{\bm \Sigma} $. Consider the $(st,s^\prime t^\prime)$ entry of $\hat{\bm \Sigma}$:
\begin{align*}
     \hat{\Sigma}_{st,s^\prime t^\prime} & = m \kappa(1-\kappa) \ip{\bm V_{st}}{\bm V_{s^\prime t^\prime}} \\
    & = m \kappa(1-\kappa) \ip{\bm o_{a_{\blocks_s}}  \odot \bm  o_{a_{\blocks_t}} - \delta(s,t) \hat{\bm e}}{\bm o_{a_{\blocks_s^\prime}}  \odot \bm  o_{a_{\blocks_t^\prime}}-\delta(s^\prime,t^\prime) \hat{\bm e}} \\
    & = m \kappa(1-\kappa) \left[ \sum_{i=1}^m \left( \bm (\bm o_{a_{\blocks_s}})_i  (\bm  o_{a_{\blocks_t}})_i -  \frac{\delta(s,t)}{m}\right) \left( (\bm o_{a_{\blocks_s^\prime}})_i   (\bm  o_{a_{\blocks_t^\prime}})_i- \frac{\delta(s^\prime,t^\prime)}{m}\right)  \right].  
\end{align*}
Note that $\bm O_i$ is a uniformly random unit vector. Hence we can compute $\E \hat{\bm \Sigma}$ using Fact \ref{fact: unit_vector_moments}. We obtain:
\begin{align*}
    \frac{\E \hat{\Sigma}_{st,s^\prime t^\prime}}{\kappa(1-\kappa)}& = \begin{cases} 2 - \frac{6}{m+2}: & s = s^\prime = t = t^\prime \\
    \frac{2}{(m-1)(m+2)}:  & s = t, s^\prime = t^\prime, s \neq s^\prime \\
    1 + \frac{2}{(m-1)(m+2)}: & s = s^\prime, t = t^\prime,  s \neq t \\ 0 : & \text{otherwise} \end{cases}.
\end{align*}
Hence, the bias term can be bounded by:
\begin{align*}
     \|\E\hat{\bm \Sigma} - \bm \Sigma \|_\fr^2 & \leq \frac{36\cdot k^4 \cdot \kappa^2 (1-\kappa)^2}{(m+2)^2}.
\end{align*}
On the other hand, applying the Poincare Inequality (Fact \ref{fact: poincare_haar}) and a tedious calculation involving 6th moments of a random unit vector (see for example Proposition 2.5 of \citet{meckes2019random}) shows that,
\begin{align*}
    \var(\hat{\Sigma}_{st,s^\prime t^\prime}) & \leq \frac{C\cdot \kappa^2(1-\kappa)^2}{m},
\end{align*}
for some universal constant $C$.
Hence,
\begin{align*}
    \E \|\hat{\bm \Sigma} - \E\hat{\bm \Sigma} \|_\fr^2 & \leq \frac{C\cdot k^4\cdot \kappa^2(1-\kappa)^2}{m},
\end{align*}
for some universal constant $C$, and consequently the claim of the lemma holds. 
\end{description}
\end{proof}


\begin{lem} \label{lemma: coupling exact form} 
 We have,
 \begin{align*}
     \E \left[ \|\bm T - \hat{\bm T} \|^2_2\right] & \leq \frac{Ck^3}{\sqrt{m}}, 
\end{align*}
for a universal constant $C$.
\end{lem}

\begin{proof}
Let $\bar {\bm b}, \hat{\bm b} \in \R^m$ be the vectors formed by  the diagonals of $\barB, \hat{\bm B}$, respectively. Define:
\begin{align*}
    p_1 & = \P( \bar{b}_1 \neq \hat{b}_1), \; p_2 = \P(\bar{b}_1 \neq \hat{b}_1, \; \bar{b}_2 \neq \hat{b}_2).
\end{align*}
We have,
\begin{align*}
    \E \left[ \|\bm T - \hat{\bm T} \|^2_2 \; | \;  \bm V \right] & =
    m \e{(\barb - \hatb)^\UT {\bm V \bm V^\UT} (\barb - \hatb)}
    \\ &
    = m \Tr \intoo{{\bm V \bm V^\UT} \e{(\barb - \hatb) (\barb - \hatb)^\UT}}
    \\ &
    = m \Tr \intoo{{\bm V \bm V^\UT} (1 - 2 \kappa)^2 \intoo{p_2 {\bm 1 \bm 1^\UT + (p_1 - p_2) \bm I_m}}}
    \\ &
    = m (1 - 2 \kappa)^2 \intoo{p_2 \norm{\bm V^\UT \bm 1}^2_2 + (p_1 - p_2) \Tr \intoo{\bm V \bm V^\UT} }.
\end{align*}
Now, since $\bm V^\UT$ has centered coordinate-wise product of columns of an orthogonal matrix we have $ \bm V^\UT \bm 1 = 0 $. Hence,
\begin{align*}
    \E \left[ \|\bm T - \hat{\bm T} \|^2_2 \; | \;  \bm V \right] &  = (p_1 - p_2) \Tr \intoo{\bm V \bm V^\UT} .
\end{align*}
Next we compute $p_1 = \P(\bar{b}_1 \neq \hat{b}_1)$. Observe that conditional on $N$, the symmetric difference $S \triangle \hat{S}$ is a uniformly random set of size $|N-n|$. Hence,
\begin{align*}
    \P(\bar{b}_1 \neq \hat{b}_1 | N) & = \P( 1 \in  S \triangle \hat{S} | N) = \frac{|n-N|}{m}.
\end{align*}
Therefore
\begin{align*}
    p_1 = \frac{\e{N - n}}{m} \leq \frac{\sqrt{{\rm Var}(N))}}{m} = \frac{\sqrt{\kappa (1 - \kappa)}}{\sqrt{m}}.
\end{align*}
Hence, we  obtain
\begin{equation}
    \E \left[ \|\bm T - \hat{\bm T} \|^2_2 |\bm V\right] \leq  \frac{(1-2\kappa)^2 }{\sqrt{m \cdot \kappa(1-\kappa)}} \cdot  \Tr(\hat{\bm \Sigma}).
\end{equation}
By Lemma \ref{lemma: asymptotic covariance} we have,
\begin{align*}
    \E \Tr(\hat{\bm \Sigma}) & \leq \E \Tr({\bm \Sigma}) + \sqrt{d \cdot \E \|\hat{\bm \Sigma} - \bm \Sigma \|_\fr^2} \\
    & \leq  C \kappa(1-\kappa) k^3.
\end{align*}
where constant $C_{\kappa, d}$ depends only on $\kappa, d$.
And hence,
\begin{align*}
     \E \left[ \|\bm T - \hat{\bm T} \|^2_2\right] & \leq \frac{Ck^3}{\sqrt{m}}, 
\end{align*}
for a universal constant $C$.
\end{proof}



\begin{lem} \label{lemma: berry_eseen} Under the assumptions and notations of Lemma \ref{lemma: asymptotic covariance} for both the subsampled Haar sensing and the subsampled Hadamard sensing models, we have, for any bounded Lipschitz function $f: \R^d \rightarrow \R$:
\begin{align} \label{eq:lemma berry eseen}
    \E\left| \E[ f(\hat{\bm T}) | \bm V] - \E f(\hat{\bm {\Sigma}}^{1/2} \bm Z) \right| \leq   \frac{C_k \cdot (\| f\|_\infty + \|f\|_{\mathsf{Lip}})}{\sqrt{m}}.
\end{align}
where $\bm Z \sim \gauss{\bm 0}{\bm I_d}$, $C_k$ is a constant depending only on $k$.
\end{lem}

\begin{proof}
Note that $\hat{\bm T} = \sqrt{m} {\bm V}^\UT \hatb$ and $ \sqrt{m} \hat{\bm \Sigma}^{\frac{-1}{2}} \bm{V}^\UT \hatb $ has the identity covariance matrix.  Hence, by the Berry-Esseen bound of \citet{bhattacharya1975errors} for any bounded and Lipschitz function $g$ we have
\begin{align} \label{eq: berry esseen normalized}
    \abs{\e{g \intoo{\hat{\bm \Sigma}^{\frac{-1}{2}}\hat{\bm T}}} - \e{g(\bm Z)}} \leq \frac{C_d \cdot \rho_3' \cdot  \intoo{\norm{g}_{\infty} + \norm{g}_{Lip}}}{\sqrt{m}},
\end{align}
where $C_d$ is a constant only dependent on $d$ and
\begin{align*}
    \rho_3' &= m^2 \sum_{i = 1}^m \e{|\hat{b}_i|^3 \cdot  \|\hat{\bm \Sigma}^{\frac{-1}{2}} \bm v_i\|^3_2 | \bm V}
    \\ &
    = m^2 \intoo{\kappa (1 - \kappa)^3 + (1 - \kappa) \kappa^3} \sum_{i
    = 1}^m { \|\hat{\bm \Sigma}^{\frac{-1}{2}} \bm v_i\|^3_2 }
    \\ &
    \leq m^2 \cdot \sqrt{d} \cdot \|\hat{\bm \Sigma}^{-\frac{1}{2}}\|_{\op}^3 \cdot (\kappa(1-\kappa)) \cdot  \sum_{i=1}^m  \|\bm v_i\|_3^3\end{align*}.

%Moreover, since $ \hat{\bm \Sigma} = m \kappa(1-\kappa) \bm V^\UT \bm V $, we can rewrite $\rho_3'$ as
%\begin{align} \label{eq:rho' definition}
%    \rho_3' 
%    = \frac{c_\kappa}{m} \sum_{i = 1}^m {\norm{\intoo{\bm V^\UT \bm V}^{\frac{-1}{2}} {\bm V^\UT} {\bm e_i}}}^3.
%\end{align}


Define $g(X) \define f \intoo{{\hat{\bm \Sigma}}^{\frac{1}{2}} {\bm X} } $, hence, $g \intoo{\hat{\bm \Sigma}^{\frac{-1}{2}} {\bm V}^\UT \hatb} = f \intoo{\hat{T}}$.  Moreover, $\norm{g}_{\infty} \leq \norm{f}_{\infty}$ and $\norm{g}_{Lip} \leq  \norm{\bm \Sigma}_{op}^{\frac{1}{2}} \norm{f}_{Lip}$. Hence we obtain:
\begin{align} \label{eq: berry_eseen_conclusion}
    &\left| \E[ f(\bm \hat{T}) | \bm V] - \E f(\hat{\bm {\Sigma}}^{1/2} \bm Z) \right|  \leq \nonumber  \\& \hspace{2cm}
    {C_d   (\kappa(1-\kappa)) \cdot  m^{\frac{3}{2}} \cdot  (\norm{f}_{\infty} + \|\hat{\bm \Sigma}\|_{\op}^{\frac{1}{2}} \norm{f}_{\mathsf{Lip}} } ) \cdot \|\hat{\bm \Sigma}^{-\frac{1}{2}}\|_{\op}^3 \cdot \sum_{i=1}^m  \|\bm v_i\|_3^3.
\end{align}
We define the event:
\begin{align*}
   \mathcal{E} \explain{def}{=} \left\{\bm V: \|\hat{\bm \Sigma} - \bm \Sigma \|_\fr^2 \leq \frac{\kappa^2(1-\kappa)^2}{4}\right\}.
\end{align*}
By Markov Inequality and Lemma \ref{lemma: asymptotic covariance}, we know that, $\P(\mathcal{E}^c) \leq Ck^4/m$ for some universal constant $C$. Hence,
\begin{align*}
     \E\left| \E[ f(\bm \hat{T}) | \bm V] - \E f(\hat{\bm {\Sigma}}^{1/2} \bm Z) \right| & \leq \frac{2 C \cdot  \|f\|_\infty \cdot  k^4}{m} + \E \left| \E[ f(\bm \hat{T}) | \bm V] - \E f(\hat{\bm {\Sigma}}^{1/2} \bm Z) \right| \Indicator{\mathcal{E}}.
\end{align*}
On the event $\mathcal{E}$ we have,
\begin{align*}
    \|\hat{\bm \Sigma}\|_{\op} & \leq \|\bm \Sigma\|_{\op} + \frac{\kappa(1-\kappa)}{2} \leq \frac{5\kappa(1-\kappa)}{2}, \\
     \|\hat{\bm \Sigma}^{-\frac{1}{2}}\|_{\op} & \leq \|{\bm \Sigma}^{-\frac{1}{2}}\|_{\op}  +  \|\hat{\bm \Sigma}^{-\frac{1}{2}} -  {\bm \Sigma}^{-\frac{1}{2}}\|_{\op} \explain{(a)}{\leq} \frac{1}{\kappa(1-\kappa)} + \frac{1}{2} \leq \frac{9}{8(\kappa(1-\kappa))}, \\
     \E\|\bm v_i\|^3  & = \sum_{j=1}^d \E |v_{ij}|^3 \explain{(b)}{\leq} \frac{Cd}{m^3}.
\end{align*}
In the step marked (a) we used the continuity estimate for matrix square root in Fact \ref{fact: matrix_sqrt}. In the step marked (b), we recalled the definition of $\bm v_i$ and used the moment bounds for a coordinate of a random unit vector from Fact \ref{fact: unit_vector_moments}. Substituting these estimates in \eqref{eq: berry_eseen_conclusion} we obtain:
\begin{align*}
    \E\left| \E[ f(\hat{\bm T}) | \bm V] - \E f(\hat{\bm {\Sigma}}^{1/2} \bm Z) \right| \leq \frac{2 C \cdot  \|f\|_\infty \cdot  k^4}{m} +  \frac{C_k \cdot (\| f\|_\infty + \|f\|_{\mathsf{Lip}})}{\sqrt{m}}.
\end{align*}
\end{proof}

Using the above lemmas, we can now provide a proof of Propositions \ref{prop: clt_hadamard} and \ref{prop: clt_random_ortho}.

\begin{proof}[Proof of Propositions \ref{prop: clt_hadamard} and \ref{prop: clt_random_ortho}]
Define the polynomial $p(\bm z)$ as:
\begin{align*}
    p(\bm z) \explain{def}{=} \prod_{\substack{s,t \in [|\pi|]\\ s \leq t \\ W_{st} (\bm w, \pi) > 0}} z_{st}^{W_{st}(\bm w, \pi)},
\end{align*}
and the indicator function:
\begin{align*}
    \Indicator{\mathcal{E}}(\bm z) & \explain{def}{=} \begin{cases} 1 : & \bm z \in \mathcal{E} \\ 0 : & \bm z \not \in \mathcal{E} \end{cases},
\end{align*}
where:
\begin{align*}
    \mathcal{E} &\explain{def}{=} \left\{ \max_{s,t} |z_{st}|  \leq \left({2048\log^3(m)} \right)^{\frac{1}{2}}\right\}.
\end{align*}
Recall that we had,
\begin{align*}
    \matmom{ \sqrt{m}\bm \Psi}{\bm w}{\pi}{\bm a} & = \prod_{\substack{s,t \in [|\pi|]\\ s \leq t \\ W_{st} (\bm w, \pi) > 0}} T_{st}^{W_{st}(\bm w, \pi)} \explain{}{=} p(\bm T),
\end{align*}
and in Lemma \ref{lemma: trace_good_event} we showed that,
\begin{align*}
    \P(\bm T \notin \mathcal{E}) & \leq \frac{C}{m^2}. 
\end{align*}
We additionally define the function $\widetilde{p}(\bm z) \explain{def}{=} p(\bm z) \Indicator{\mathcal{E}}(\bm z)$. observe that:
\begin{align*}
    \|\widetilde{p}\|_\infty & \leq \left({2048\log^3(m)} \right)^{\frac{\|\bm w\|}{2}}, \; \|\widetilde{p}\|_\mathsf{Lip}  \leq \|\bm w\| \left({2048\log^3(m)} \right)^{\frac{\|\bm w\|}{2}}.
\end{align*}
Let $\bm Z \sim \gauss{\bm 0}{\bm I_d}$. Then, we can write:
\begin{align*}
    &\left| \E p(\bm T) - \E p(\bm \Sigma^{\frac{1}{2}} \bm Z) \right|  \leq  \left| \E \widetilde{p}(\bm T) - \E \widetilde{p}(\bm \Sigma^{\frac{1}{2}} \bm Z) \right|  + |\E p(\bm T) \Indicator{\mathcal{E}^c}(\bm T)| + |\E p(\bm T) \Indicator{\mathcal{E}^c}(\bm \Sigma^{\frac{1}{2}} Z)| \\
     &\leq\underbrace{\left| \E \widetilde{p}(\bm T) - \E \widetilde{p}(\hat{\bm T}) \right|}_{\mathsf{(I)}}+  \underbrace{\left| \E \widetilde{p}(\bm T) - \E \widetilde{p}(\hat{\bm \Sigma}^{\frac{1}{2}} \bm Z) \right|}_{\mathsf{(II)}} + \underbrace{\left| \E \widetilde{p}({\bm \Sigma}^{\frac{1}{2}} \bm Z) - \E \widetilde{p}(\hat{\bm \Sigma}^{\frac{1}{2}} \bm Z) \right|}_{\mathsf{(III)}}  \\&\hspace{7cm} + \underbrace{|\E p(\bm T) \Indicator{\mathcal{E}^c}(\bm T)|}_{\mathsf{(IV)}} + \underbrace{|\E p( {\bm \Sigma}^{\frac{1}{2}}\bm Z) \Indicator{\mathcal{E}^c}(\bm \Sigma^{\frac{1}{2}}\bm  Z)|}_{\mathsf{(V)}}.
\end{align*}
We control each of these terms separately.
\begin{description}
\item [Analysis of $(\mathsf{I})$:] In order to control $\mathsf{I}$ observe that:
\begin{align*}
    \mathsf{(I)} & \leq \|\widetilde{p}\|_\mathsf{Lip} \E \|\bm T - \hat{\bm T}\|_2  \\& \leq \|\widetilde{p}\|_\mathsf{Lip} \cdot (\E \|\bm T - \hat{\bm T}\|_2^2)^{\frac{1}{2}}\\  & \leq C \cdot \|\bm w\|\cdot  \left({2048\log^3(m)} \right)^{\frac{\|\bm w\|}{2}} \cdot \frac{\sqrt{k^3}}{m^\tbd}.
\end{align*}
In the last step, we appealed to Lemma \ref{lemma: coupling exact form}.
\item [Analysis of $(\mathsf{II})$:] In order to control $\mathsf{I}$, recall that:
\begin{align*}
    \|\widetilde{p}\|_\infty & \leq \left({2048\log^3(m)} \right)^{\frac{\|\bm w\|}{2}}, \; \|\widetilde{p}\|_\mathsf{Lip}  \leq \|\bm w\| \left({2048\log^3(m)} \right)^{\frac{\|\bm w\|}{2}}.
\end{align*}
Hence, by Lemma \ref{lemma: berry_eseen} we have,
\begin{align*}
    \mathsf{(II)} & \leq \frac{C_k \cdot ({2048\log^3(m)} )^{\frac{\|\bm w\|}{2}} (1 + \|\bm w\|)}{\sqrt{m}}.
\end{align*}
\item [Analysis of $(\mathsf{III})$: ]Again using the Lipchitz bound on $\widetilde{p}$ we have,
\begin{align*}
    (\mathsf{III}) & \leq \E |\widetilde{p}({\bm \Sigma}^{\frac{1}{2}} \bm Z) -  \widetilde{p}(\hat{\bm \Sigma}^{\frac{1}{2}} \bm Z)| \\
    & \leq \|\bm w\| \left({2048\log^3(m)} \right)^{\frac{\|\bm w\|}{2}} \cdot \E \|(\hat{\bm \Sigma}^{\frac{1}{2}} - {\bm \Sigma}^{\frac{1}{2}}) \bm Z\|_2 \\
    & \leq \|\bm w\| \left({2048\log^3(m)} \right)^{\frac{\|\bm w\|}{2}} \cdot \sqrt{\E \|(\hat{\bm \Sigma}^{\frac{1}{2}} - {\bm \Sigma}^{\frac{1}{2}}) \bm Z\|^2_2} \\
    & \leq \|\bm w\| \left({2048\log^3(m)} \right)^{\frac{\|\bm w\|}{2}} \cdot \sqrt{\E \|\hat{\bm \Sigma}^{\frac{1}{2}} - {\bm \Sigma}^{\frac{1}{2}} \|^2_\fr} \\
    &\explain{(a)}{\leq} \|\bm w\| \left({2048\log^3(m)} \right)^{\frac{\|\bm w\|}{2}} \cdot  \frac{k^2}{\lambda_{\max}(\bm \Sigma)} \cdot \E \|\hat{\bm \Sigma} - \bm \Sigma\|_\fr^2 \\
    & \explain{(b)}{\leq} \frac{C \cdot k^6 \cdot \|\bm w\| ({2048\log^3(m)} )^{\frac{\|\bm w\|}{2}}}{m}.
\end{align*}
In the step marked (a) we used the fact that the continuity estimate for matrix square roots given in Fact \ref{fact: matrix_sqrt}. In the step marked (b) we recalled the definition of $\bm \Sigma$ and observed that $\lambda_{\max}(\bm \Sigma) \geq \kappa(1-\kappa)$ for the subsampled Haar and the Hadamard sensing model. We also used the bound on $\E \|\hat{\bm \Sigma} - \bm \Sigma \|_{\fr}^2$ obtained in Lemma \ref{lemma: asymptotic covariance}.
\item  [Analysis of $(\mathsf{IV})$: ] We can control $(\mathsf{III})$ as follows:
\begin{align*}
    (\mathsf{IV}) & \leq \sqrt{\E p^2(\bm T) } \cdot \sqrt{\P(\bm T \not \in \mathcal{E})} \\
    & \explain{(c)}{\leq} \frac{C  \sqrt{\E \matmom{\sqrt{m}\bm \Psi}{2 \bm w}{\pi}{\bm a}}}{m} \\
    & \explain{(d)}\leq \frac{(C\|\bm w\| \log^2(m))^{\frac{\|\bm w\|}{2}}}{m}
\end{align*}
In the step marked (c) we recalled that $\P(\bm T \notin \mathcal{E}) \leq C/m^2$ and expressed $p^2(\bm T)$ as a matrix moment. In the step marked (d) we used the bounds on matrix moments obtained in Lemma \ref{lemma: matrix_moment_ub}.
\item  [Analysis of $(\mathsf{IV})$: ] We recall that $\bm \Sigma$ was a diagonal matrix with $|\Sigma_{ii}| \leq 2 \kappa(1-\kappa) \leq 1$. Hence,
\begin{align*}
    (\mathsf{V}) & \leq \sqrt{\E p^2(\bm \Sigma^{\frac{1}{2}})} \cdot \sqrt{\P (\bm \Sigma^{\frac{1}{2}} \bm Z \notin \mathcal{E})} \\
    & \explain{(e)}{\leq} \frac{k\|\bm w\|^{\frac{\|\bm w\|}{2}}}{m}.
\end{align*}
In the step marked (e) we used standard moment and tail bounds on Gaussian random variables. 
\end{description}
Combining the bounds on $\mathsf{I}-\mathsf{V}$ immediately yields the claims of Proposition \ref{prop: clt_hadamard} and \ref{prop: clt_random_ortho}.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% APPENDIX-QF%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Missing Proofs from Section \ref{section: qf_proof}}
\label{appendix: qf}

\subsection{Proof of Lemma \ref{lemma: continuity_qf}}
\label{proof: continuity_qf}
\begin{proof}[Proof of Lemma \ref{lemma: continuity_qf}] We will assume that $\altprod$ is of Type 1 (the proof of the other types is analogous): 
\begin{align*}
    \altprod(\bm \Psi, \bm Z) = p_1(\bm \Psi) q_1(\bm Z) p_2(\bm \Psi) \cdots  q_{k-1}(\bm Z) p_k(\bm \Psi).
\end{align*}
% \begin{enumerate}
    % \item (Continuity with respect to $\bm z$) 
    Define for any $i \in [k]$:
    \begin{align*}
        \altprod_0 & \explain{def}{=} p_1(\bm \Psi) q_1(\diag{\bm z}) p_2(\bm \Psi) \cdots  q_{k-1}(\diag{\bm z}) p_k(\bm \Psi), \\
        \altprod_i & \explain{def}{=} p_1(\bm \Psi) q_1(\diag{\widetilde{\bm z}})  \cdots  q_i(\diag{\widetilde{\bm z}}) p_{i+1}(\bm \Psi) q_{i+1}(\diag{{\bm z}}) \cdots q_{k-1}(\diag{\bm z}) p_k(\bm \Psi).
    \end{align*}
    where $\bm \Psi = \bm U \barB \bm U^\UT$.
    Observe that we can write:
    \begin{align*}
        &\bm z^\UT \altprod(\bm U \barB \bm U^\UT, \diag{\bm z}) \bm z - \widetilde{\bm z}^{\UT} \altprod(\bm U \barB \bm U^\UT, \diag{\widetilde{\bm z}}) \widetilde{\bm z}  = \bm z^\UT \altprod_0 \bm z - \widetilde{\bm z}^\UT \altprod_{k-1} \widetilde{\bm z} \\
        & = \bm z^\UT \altprod_0 \bm z - \bm z^\UT \altprod_{k-1} \bm z + \bm z^\UT \altprod_{k-1} \bm z +  \widetilde{\bm z}^\UT \altprod_{k-1} \widetilde{\bm z} \\
        & = \left(\sum_{i=0}^{k-2} \bm z^\UT (\altprod_i - \altprod_{i+1}) \bm z \right) + \ip{\altprod_{k-1}}{\bm z \bm z^\UT - \widetilde{\bm z}\widetilde{\bm z}^\UT}. 
    \end{align*}
    We bound each of these terms separately. First observe that:
    \begin{align*}
        |\bm z^\UT (\altprod_i - \altprod_{i+1}) \bm z| & \leq \|\bm z\|_2^2 \cdot \| \altprod_i - \altprod_{i+1}\|_\op \\
        & \leq  C(\altprod) \cdot  \|\bm z\|_2^2 \cdot \|\bm z - \widetilde{\bm z}\|_\infty.
    \end{align*}
    Next we note that,
    \begin{align*}
        |\ip{\altprod_{k-1}}{\bm z \bm z^\UT - \widetilde{\bm z}\widetilde{\bm z}^\UT}| & \leq 2\|\altprod_{k-1}\|_\op \cdot \| \bm z \bm z^\UT - \widetilde{\bm z}\widetilde{\bm z}^\UT\|_\op \\
        & = C(\altprod) \cdot \|\bm z - \widetilde{\bm z}\|_2 \cdot (\|\bm z\|_2 + \|\widetilde{\bm z}\|_2).
    \end{align*}
    This gives is the estimate:
    \begin{align*}
         &\left| \frac{\bm z^\UT \altprod(\bm U \barB \bm U^\UT, \diag{\bm z}) \bm z}{m}  - \frac{\widetilde{\bm z}^{\UT} \altprod(\bm U \barB \bm U^\UT, \diag{\widetilde{\bm z}}) \widetilde{\bm z}}{m}   \right|  \leq \\ & \hspace{5cm} \frac{C(\altprod)}{m} \cdot \left(  \|\bm z\|_2^2 \cdot \|\bm z - \widetilde{\bm z}\|_\infty +   \|\bm z - \widetilde{\bm z}\|_2 \cdot (\|\bm z\|_2 + \|\widetilde{\bm z}\|_2) \right),
    \end{align*}
    where $C(\altprod)$ denotes a finite constant depending only on the $\|\|_\infty$ norms and Lipchitz constants of the functions appearing in $\altprod$.
% \item (Continuity with respect to $\bm U$) Let $\bm \Psi = \bm U \barB \bm U^\UT$, $\widetilde{\bm \Psi} = \widetilde{\bm U} \barB \widetilde{\bm U}^\UT, \bm Z = \diag{\bm z}$. In analogy with the previous part, we define:
% \begin{align*}
%         \altprod_0 & \explain{def}{=} p_1(\bm \Psi) q_1(\bm Z) p_2(\bm \Psi) \cdots  q_{k-1}(\bm Z) p_k(\bm \Psi), \\
%         \altprod_i & \explain{def}{=} p_1(\widetilde{\bm \Psi}) q_1(\bm Z) \cdots  p_{i}(\widetilde{\bm \Psi}) q_i(\bm Z) p_{i+1}(\bm \Psi) \cdots  q_{k-1}(\bm Z) p_k(\bm \Psi), \; \forall \; i \; \in \;[k+1].
% \end{align*}
% With this notation, we can write,
% \begin{align*}
%       \bm z^\UT \altprod(\bm U \barB \bm U^\UT, \diag{\bm z}) \bm z -\bm z^\UT \altprod(\widetilde{\bm U} \barB \widetilde{\bm U}^\UT, \diag{\bm z}) \bm z   & = \sum_{i=0}^{k-1} \bm z^\UT (\altprod_{i} - \altprod_{i+1}) \bm z.
% \end{align*}
% We will bound each term individually. First observe that:
% \begin{align*}
%     \altprod_{i-1} - \altprod_{i} & = \mathcal{L}_i \cdot (p_i(\bm \Psi) - p_i(\widetilde{\bm \Psi})) \cdot \mathcal{R}_i,\\ \mathcal{L}_i &\explain{def}{=} p_1(\widetilde{\bm \Psi}) q_1(\bm Z) \cdots  p_{i-1}(\widetilde{\bm \Psi}) q_{i-1}(\bm Z),\\
%     \mathcal{R}_i & \explain{def}{=} q_{i}(\bm Z) p_{i+1}(\bm \Psi) \cdots q_{k-1}(\bm Z) p_k(\bm \Psi).
% \end{align*}
% Hence,
% \begin{align*}
%     |\bm z^\UT (\altprod_{i-1} - \altprod_{i}) \bm z | & = | \bm z^\UT \mathcal{L}_i \cdot (p_i(\bm \Psi) - p_i(\widetilde{\bm \Psi})) \cdot \mathcal{R}_i \bm z| \\
%     & \leq \|p_i(\bm \Psi) - p_i(\widetilde{\bm \Psi})\|_\op  \|\mathcal{L}_i\|_\op \|\mathcal{R}_i\|_\op \|\bm z\|^2 \\
%     & \leq C(\altprod) \cdot \|\bm z\|^2 \cdot \|p_i(\bm \Psi) - p_i(\widetilde{\bm \Psi})\|_\op \\
%     & \leq C(\altprod) \cdot \|\bm z\|^2 \cdot \|p_i(\bm \Psi) - p_i(\widetilde{\bm \Psi})\|_\fr \\
%     & = C(\altprod) \cdot \|\bm z\|^2 \cdot\left( \|\bm U p_i(\barB) \cdot( \bm U^\UT - \widetilde{\bm U}^\UT)\|_\fr + \|(\bm U - \widetilde{\bm U}) \cdot p_i(\barB) \widetilde{\bm U}^\UT\|_\fr  \right) \\
%     & \leq C(\altprod) \cdot \|\bm z\|^2 \cdot \|\bm U - \widetilde{\bm U}\|_\fr.
% \end{align*}
% Hence we obtain the estimate:
% \begin{align*}
%     \frac{1}{m} \left| \bm z^\UT \altprod(\bm U \barB \bm U^\UT, \diag{\bm z}) \bm z -\bm z^\UT \altprod(\widetilde{\bm U} \barB \widetilde{\bm U}^\UT, \diag{\bm z}) \bm z  \right| & \leq \frac{C(\altprod) \cdot \|\bm z\|^2}{m} \cdot \|\bm U - \widetilde{\bm U}\|_\fr,
% \end{align*}
% where $C(\altprod)$ denotes a finite constant depending only on the $\|\cdot\|_\infty$ norms and Lipchitz constants of the functions appearing in $\altprod$.
% \end{enumerate}
\end{proof}

\subsection{Proof of Lemma \ref{lemma : qf_variance_normalization}}
\label{proof: qf_variance_normalization}
\begin{proof}[Proof of Lemma \ref{lemma : qf_variance_normalization}] Using the continuity estimate from Lemma \ref{lemma: continuity_qf} we know that on the event $\mathcal{E}$,
\begin{align*}
     &\left| \frac{\bm z^\UT \altprod(\bm \Psi, \bm Z) \bm z}{m}  - \frac{\widetilde{\bm z}^{\UT} \altprod(\bm\Psi, \widetilde{\bm Z}) \widetilde{\bm z}}{m}   \right|  \leq \frac{C(\altprod)}{m} \cdot \left(  \|\bm z\|_2^2 \cdot \|\bm z - \widetilde{\bm z}\|_\infty +   \|\bm z - \widetilde{\bm z}\|_2 \cdot (\|\bm z\|_2 + \|\widetilde{\bm z}\|_2) \right) \\
     & \leq \frac{C(\altprod)}{m} \cdot \left(  \|\bm z\|_2^2 \cdot \|\bm z\|_\infty +   \|\bm z\|_2 \cdot (\|\bm z\|_2 + \|\widetilde{\bm z}\|_2) \right) \cdot \left( \max_{i \in [m]} \left| \frac{1}{\sigma_i} - 1 \right| \right) \\
     & \leq \frac{C(\altprod)}{m \kappa } \cdot \left(  \|\bm z\|_2^2 \cdot \|\bm z\|_\infty +   \|\bm z\|_2 \cdot (\|\bm z\|_2 + \|\widetilde{\bm z}\|_2) \right) \cdot \sqrt{\frac{\log^{3}(m)}{m}} 
\end{align*}
Hence,
\begin{align*}
    &\left| \E \frac{\bm z^\UT \altprod(\bm \Psi, \bm Z) \bm z}{m}  - \E \frac{\widetilde{\bm z}^{\UT} \altprod(\bm\Psi, \widetilde{\bm Z}) \widetilde{\bm z}}{m} \Indicator{\mathcal{E}} \right| \leq \left| \E \frac{\bm z^\UT \altprod(\bm \Psi, \bm Z) \bm z}{m} \Indicator{\mathcal{E}^c}\right|  \\ &\hspace{4cm}+ \frac{C(\altprod)\log^{\frac{3}{2}}(m)}{m\sqrt{m} \kappa } \cdot \left(  \E\|\bm z\|_2^2 \cdot \|\bm z\|_\infty +   \E\|\bm z\|_2 \cdot (\|\bm z\|_2 + \|\widetilde{\bm z}\|_2) \right).
\end{align*}
Observe that $\bm z^\UT \altprod \bm z \leq  \|\altprod\|_\op \|\bm z\|^2 \leq C(\altprod) \|\bm z\|^2_2 \leq C(\altprod) \|\bm x\|^2_2 $. 
Hence,
\begin{align*}
    \left| \E \frac{\bm z^\UT \altprod(\bm \Psi, \bm Z) \bm z}{m} \Indicator{\mathcal{E}^c}\right| & \leq C(\altprod)\frac{\sqrt{\E\|\bm x\|^4_2 \cdot \P(\mathcal{E}^c)}}{m} \leq \frac{C(\altprod) \sqrt{\P(\mathcal{E}^c)}}{\kappa^2} \rightarrow 0, \\
    \E\|\bm z\|^2_2 + \E \|\bm z\|_2 \|\widetilde{\bm z}\|_2  & \leq 2\E \|\bm z\|_2^2 + \E \|\widetilde{\bm z}\|_2^2 \leq 2\E \|\bm x\|_2^2 + \E \|\widetilde{\bm z}\|_2^2 = \frac{2m}{\kappa} + m, \\
    \E\|\bm z\|_2^2 \cdot \|\bm z\|_\infty & \leq m \E \|\bm z\|_\infty^3 \leq m \left(\E \|\bm z\|^9_9 \right)^{\frac{1}{3}} \leq C m^{\frac{4}{3}}.
\end{align*}
This gives us,
\begin{align*}
     \left| \E \frac{\bm z^\UT \altprod(\bm \Psi, \bm Z) \bm z}{m}  - \E \frac{\widetilde{\bm z}^{\UT} \altprod(\bm\Psi, \widetilde{\bm Z}) \widetilde{\bm z}}{m} \Indicator{\mathcal{E}} \right|  \rightarrow 0,
\end{align*}
and hence we have shown,
\begin{align*}
    \lim_{m \rightarrow \infty} \frac{\E \bm z^\UT \altprod(\bm \Psi, \bm Z) \bm z}{m}&=\lim_{m \rightarrow \infty}\E \frac{\widetilde{\bm z}^{\UT} \altprod(\bm\Psi, \widetilde{\bm Z}) \widetilde{\bm z}}{m} \Indicator{\mathcal{E}},
\end{align*}
provided the latter limit exists.
\end{proof}

\subsection{Proof of Lemma \ref{lemma: qf_mehler_conclusion}}
\label{proof: qf_mehler_conclusion}
\begin{proof}[Proof of Lemma \ref{lemma: qf_mehler_conclusion}] Recall that:
\begin{align*}
        \widetilde{z}_{a_1} \widetilde{z}_{a_{k+1}}\prod_{i=1}^k q_i(\widetilde{z}_{a_i}) & = Q_\firstfnc(\widetilde{z}_{a_1}) \cdot  Q_\lastfnc(\widetilde{z}_{a_{k+1}})  \left( \prod_{i \in \singleblks{\pi}} q_{i-1}(\widetilde{z}_{a_i}) \right)  \prod_{i=1}^{|\pi| - |\singleblks{\pi}| - 2} (Q_{\blocks_i}(z_{a_{\blocks_i}}) + \mu_{\blocks_i})
\end{align*}
Hence,
    \begin{align}
        &\E[ \widetilde{z}_{a_1} q_1(\widetilde{z}_{a_2}) q_2(\widetilde{z}_{a_3}) \cdots q_{k-1}(\widetilde{z}_{a_k})  \widetilde{z}_{a_{k+1}} |  \bm A ]   = \nonumber \\ & \sum_{V \subset [|\pi| - |\singleblks{\pi}| - 2] }  \E\left[ Q_\firstfnc(\widetilde{z}_{a_1})   Q_\lastfnc(\widetilde{z}_{a_{k+1}})  \left( \prod_{i \in \singleblks{\pi}} q_{i-1}(\widetilde{z}_{a_i}) \right)  \prod_{i \in V} (Q_{\blocks_i}(\widetilde{z}_{a_{\blocks_i}}))   \bigg| \bm A \right]  \left( \prod_{i \notin V} \mu_{\blocks_i} \right) \label{eq: qf_lemma_firstmom_Vexpansion}
    \end{align}
    We now apply Mehler's formula to estimate the above conditional expectations. We first check the conditions for Mehler's formula:
    \begin{enumerate}
        \item The random variables $\widetilde{\bm z}$ are marginally $\gauss{0}{1}$. Define $\bm \Sigma = \E [\widetilde{\bm z} \widetilde{\bm z}^\UT | \bm A]$. $\bm{\widetilde{z}}$ and are weakly correlated on the event $\mathcal{E}$ since:
        \begin{align*}
            \max_{i \neq j} |\Sigma_{ij}| & = \left| \frac{(\bm A \bm A^\UT)_{ij}/\kappa}{\sigma_i \sigma_j} \right| \\
            & = \left| \frac{(\bm\Psi)_{ij}/\kappa}{\sigma_i \sigma_j} \right| \\
            & \leq C\sqrt{\frac{\log^{3}(m)}{m \kappa^2}}, \; \text{for $m$ large enough},
        \end{align*}
        where $C$ denotes a universal constant. 
        \item Let $S \subset [m]$ with $|S| \leq k+2$. Let $\bm \Sigma_{S,S}$ denote the principal submatrix of $\bm \Sigma $ formed by picking rows and columns in $S$. Then by Gershgorin's Circle theorem, on the event $\mathcal{E}$,
        \begin{align*}
            \lambda_{\min}(\bm \Sigma) & \geq 1 - (k+1) \max_{i \neq j} | \Sigma_{ij}| \\
            & \geq 1 - C(k+1)\sqrt{\frac{\log^{3}(m)}{m \kappa^2}}\\
            & \geq \frac{1}{2}, \; \text{ for $m$ large enough}.
        \end{align*}
        \item Note that for $\xi \sim \gauss{0}{1}$, we have, 
        \begin{align*}
            &\E Q_\firstfnc(\xi) = 0, \; \E Q_\lastfnc(\xi) = 0 \; \text{ (Since they are odd functions, see \eqref{eq: q_block_first}, \eqref{eq: q_block_last})}, \\
            &\E q_{i-1}(\xi) = \E \xi q_{i-1}(\xi) = 0 \; \forall \; i \in \singleblks{\pi} \; \text{ (They are centered, even functions, see Def. \ref{def: alternating_product})}, \\
            & \E Q_{\blocks_i}(\xi) = \E \xi Q_{\blocks_i}(\xi) = 0 \; \forall \; i \; \in \; [|\pi| - |\singleblks{\pi}| - 2] \; \text{ (See \eqref{eq: q_block})} 
        \end{align*}
        Hence applying the first non-zero term in Mehler's Expansion (Proposition \ref{proposition: mehler}) of the conditional expectation:
        \begin{align*}
            \E\left[ Q_\firstfnc(\widetilde{z}_{a_1}) \cdot  Q_\lastfnc(\widetilde{z}_{a_{k+1}}) \cdot \left( \prod_{i \in \singleblks{\pi}} q_{i-1}(\widetilde{z}_{a_i}) \right) \cdot \prod_{i \in V} (Q_{\blocks_i}(\widetilde{z}_{a_{\blocks_i}}))   \bigg| \bm A \right]
        \end{align*}has total weight $\|\bm w\|$ given by:
        \begin{align*}
            \|\bm w\| & \geq  \frac{1 + 1 + 2 |\singleblks{\pi}| + 2 |V|}{2} = 1 + |\singleblks{\pi}| + |V|.
        \end{align*}
    \end{enumerate}
     Hence, by Proposition \ref{proposition: mehler} we have,
        \begin{align}
             &\Indicator{\mathcal{E}} \cdot \left| \E\left[ Q_\firstfnc(\widetilde{z}_{a_1}) \cdot  Q_\lastfnc(\widetilde{z}_{a_{k+1}}) \cdot \left( \prod_{i \in \singleblks{\pi}} q_{i-1}(\widetilde{z}_{a_i}) \right) \cdot \prod_{i \in V} (Q_{\blocks_i}(\widetilde{z}_{a_{\blocks_i}}))   \bigg| \bm A \right] \right|  \nonumber \\& \hspace{3cm} \leq  C(\altprod) (\max_{i \neq j} | \Sigma_{i,j} |)^{1 + |\singleblks{\pi}| + |V|} 
             \leq C(\altprod) \cdot \left( \frac{\log^2(m)}{m \kappa^2} \right)^{\frac{1 + |\singleblks{\pi}| + |V|}{2}}, \label{eq: mehler_conclusion_notimp}
        \end{align}
        where $C(\altprod)$ denotes a finite constant depending only on the functions $q_{1:k}$. When $V = \emptyset$ we will also need to estimate the leading order term more accurately. Define,
        \begin{align*}
            \weightedGnum{\pi}{1} & \explain{def}{=} \left\{\bm w \in \weightedG{k+1}: \degree_1(\bm w) = 1, \; \degree_{k+1}(\bm w) = 1, \; \degree_i(\bm w) = 2 \; \forall \; i \; \in \; \singleblks{\pi}, \right.\\ &\hspace{6cm} \left.\degree_i(\bm w) = 0 \; \forall \; i \; \notin \; \{1,k+1\} \cup \singleblks{\pi} \right\}.
        \end{align*}
    By Mehler's formula, on the event $\mathcal{E}$, we have:
    \begin{align*}
        & \left| \E\left[ Q_\firstfnc(\widetilde{z}_{a_1}) \cdot  Q_\lastfnc(\widetilde{z}_{a_{k+1}}) \cdot \left( \prod_{i \in \singleblks{\pi}} q_{i-1}(\widetilde{z}_{a_i}) \right)   \bigg| \bm A \right] - \sum_{\bm w \in \weightedGnum{\pi}{1}} \hat{\coeff}(\bm w,\bm \Psi) \cdot \matmom{\bm \Psi}{\bm w}{\pi}{\bm a}  \right| \\
             &\hspace{8cm }  \leq C(\altprod) \cdot \left( \frac{\log^3(m)}{m \kappa^2} \right)^{\frac{2 + |\singleblks{\pi}|}{2}},
    \end{align*}
    where,
    \begin{align*}
        \hat{\coeff}(\bm w, \bm \Psi) & = \frac{1}{\bm w!} \cdot \left(\prod_{i=1}^{k+1} \frac{1}{\sigma_{a_i}^{\degree_i(\bm w)}} \right) \cdot \left(\hat{Q}_\firstfnc(1) \hat{Q}_\lastfnc(1) \prod_{i \in \singleblks{\pi}} \hat{q}_{i-1}(2)   \right) \frac{1}{\kappa^{\|\bm w\|}}, 
    \end{align*}
    and $\matmom{\bm \Psi}{\bm w}{\pi}{\bm a}$ are matrix moments as defined in Definition \ref{def: matrix moment}. Note that the coefficients $\hat{\coeff}(\bm w, \bm \Psi)$ depend on $\bm \Psi$ since,
    \begin{align*}
        \sigma_i^2 & = 1 + \frac{\bm \Psi_{ii}}{\kappa},
    \end{align*}
    but we can remove this dependence. On the event $\mathcal{E}$, note that,
    \begin{align*}
        \max_{i \in [m]} |\sigma_{ii}^2 - 1| & \leq C \sqrt{\frac{\log^3(m)}{m \kappa^2}}.
    \end{align*}
    Hence defining:
    \begin{align*}
        \hat{\coeff}(\bm w, \pi) & = \frac{1}{\bm w!} \cdot  \left(\hat{Q}_\firstfnc(1) \hat{Q}_\lastfnc(1) \prod_{i \in \singleblks{\pi}} \hat{q}_{i-1}(2)   \right) \frac{1}{\kappa^{\|\bm w\|}}, 
    \end{align*}
    we have, for $m$ large enough and on the event $\mathcal{E}$,
    \begin{align*}
        |\hat{\coeff}(\bm w, \pi) - \hat{\coeff}(\bm w, \bm \Psi)| & \leq  C_k \sqrt{\frac{\log^3(m)}{m \kappa^2}}.
    \end{align*}
    Furthermore, we have the estimate,
    \begin{align*}
        |\matmom{\bm \Psi}{\bm w}{\pi}{\bm a}| & \leq (\max_{i,j} |\Psi_{ij}| )^{\|\bm w\|_1} \\
     & \explain{(a)}{\leq} C\left( \frac{\log^3(m)}{m \kappa^2} \right)^{\frac{1 + |\singleblks{\pi}|}{2}},
    \end{align*}
    where in the step (a), we used the definition of the event $\mathcal{E}$ in \eqref{eq: good_event_qf_firstmom} and the fact that $\|\bm w\| = 1 + |\singleblks{\pi}|$ for any $\bm w \in \weightedGnum{\pi}{1}$. Hence we obtain, on the event $\mathcal{E}$,
    \begin{align*}
        &\left| \E\left[ Q_\firstfnc(\widetilde{z}_{a_1}) \cdot  Q_\lastfnc(\widetilde{z}_{a_{k+1}}) \cdot \left( \prod_{i \in \singleblks{\pi}} q_{i-1}(\widetilde{z}_{a_i}) \right)   \bigg| \bm A \right] - \sum_{\bm w \in \weightedGnum{\pi}{1}} \hat{\coeff}(\bm w, \pi) \cdot \matmom{\bm \Psi}{\bm w}{\pi}{\bm a}  \right| \nonumber \\
             &\hspace{8cm }  \leq C(\altprod) \cdot \left( \frac{\log^3(m)}{m \kappa^2} \right)^{\frac{2 + |\singleblks{\pi}|}{2}}.
    \end{align*}
    Combining this estimate with \eqref{eq: qf_lemma_firstmom_Vexpansion} and \eqref{eq: mehler_conclusion_notimp} gives us:
    \begin{subequations}
    \begin{align*}
        &\Indicator{\mathcal{E}} \cdot \left| \E[ \widetilde{z}_{a_1} q_1(\widetilde{z}_{a_2}) q_2(\widetilde{z}_{a_3}) \cdots q_{k-1}(\widetilde{z}_{a_k})  \widetilde{z}_{a_{k+1}} |  \bm A ] - \sum_{\bm w \in \weightedGnum{\pi}{1}} {\coeff}(\bm w, \pi) \cdot \matmom{\bm \Psi}{\bm w}{\pi}{\bm a}  \right| \nonumber \\
             &\hspace{8cm }  \leq C(\altprod) \cdot \left( \frac{\log^3(m)}{m \kappa^2} \right)^{\frac{2 + |\singleblks{\pi}|}{2}},
    \end{align*}
    where
    \begin{align*}
        {\coeff}(\bm w, \pi) & = \frac{1}{{\kappa^{\|\bm w\|}} \bm w!}  \cdot \left(\hat{Q}_\firstfnc(1) \hat{Q}_\lastfnc(1) \prod_{i \in \singleblks{\pi}} \hat{q}_{i-1}(2)   \right)  \cdot \left( \prod_{i \in [|\pi| - |\singleblks{\pi}| - 2]} \mu_{\blocks_i} \right)
    \end{align*}
    \begin{align*}
            \weightedGnum{\pi}{1} & \explain{def}{=} \left\{\bm w \in \weightedG{k+1}: \degree_1(\bm w) = 1, \; \degree_{k+1}(\bm w) = 1, \; \degree_i(\bm w) = 2 \; \forall \; i \; \in \; \singleblks{\pi}, \right. \nonumber\\ &\hspace{6cm} \left.\degree_i(\bm w) = 0 \; \forall \; i \; \notin \; \{1,k+1\} \cup \singleblks{\pi} \right\},
        \end{align*}
    %\label{eq: mehler_conclusion_imp}
    \end{subequations}
    and $C(\altprod)$ denotes a constant depending only on the functions appearing in $\altprod$ and $k$. This was precisely the claim of Lemma \ref{lemma: qf_mehler_conclusion}.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% APPENDIX-MEHLER%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Proposition \ref{proposition: mehler}}
\label{appendix: mehler}
\begin{proof}[Proof of Proposition \ref{proposition: mehler}]
Let $\gpdf{\bm z}{\bm \Sigma}$ denote the density of a $k$ dimensional zero mean Gaussian vector with positive definite covariance matrix $\bm \Sigma$ i.e. $\bm z \sim \gauss{\bm 0}{\bm \Sigma}$.  Suppose that $\Sigma_{ii} = 1 \; \forall  \; i \in [k]$. In this situation \citet{slepian1972symmetrized} has found an explicit expression for the Taylor series expansion of $\gpdf{\bm z}{\bm \Sigma}$ around $\bm \Sigma = \bm I_k$ given by:
\begin{align*}
    {\gpdf{\bm z}{\bm \Sigma}} & = \sum_{\bm w \in \weightedG{k}} \frac{D^{\bm w}_{\bm \Sigma} \;  \psi(\bm z; \bm I_k)}{\bm w !} \cdot \left( \prod_{i<j} \Sigma_{ij}^{w_{ij}} \right),
\end{align*}
where $D^{\bm w}_{\bm \Sigma} \; \psi(\bm z; \bm I_k)$ denotes the derivative:
\begin{align*}
    D^{\bm w}_{\bm \Sigma} \;  \psi(\bm z; \bm I_k) & \explain{def}{=} \frac{\partial^{\|\bm w\|}}{\partial \Sigma_{12}^{w_{12}} \; \partial \Sigma_{13}^{w_{13}}\cdots \partial \Sigma_{23}^{w_{23}}\; \partial \Sigma_{24}^{w_{24}} \cdots \partial \Sigma_{k-1,k}^{w_{k-1,k}}} \;  \psi(\bm z; \bm \Sigma) \bigg|_{\bm \Sigma = \bm I_k} \\&=  \left(\prod_{i=1}^k   H_{\degree_i(\bm w)}(z_i) \right) \cdot \gpdf{\bm z}{\bm  I_k}.
\end{align*}
We intend to integrate the Taylor series for $\gpdf{\bm z}{\bm \Sigma}$ to obtain the expansion for the expectation in Proposition \ref{proposition: mehler}. In order to do so we need to understand the truncation error in the Taylor Series. By Taylors Theorem, we know that:
\begin{align}
    \gpdf{\bm z}{\bm \Sigma} -  \sum_{\bm w \in \weightedG{k}: \|\bm w\| \leq t} \frac{D^{\bm w}_{\bm \Sigma} \; \psi(\bm z; \bm I_k)}{\bm w !} \cdot \left( \prod_{i<j} \Sigma_{ij}^{w_{ij}} \right)  & = \sum_{\bm w \in \weightedG{k}: \|\bm w\| = t+1} \frac{D^{\bm w}_{\bm \Sigma} \; \gpdf{\bm z}{\bm \Sigma_\gamma}}{\bm w!} \cdot \bm \Sigma^{\bm w}, \label{eq: taylors_thm}
\end{align}
where $\bm \Sigma_\gamma = \gamma \bm \Sigma + (1-\gamma) \bm I_k$ for some $\gamma \in (0,1)$. \citeauthor{slepian1972symmetrized} has further showed the following remarkable identity:
\begin{align*}
    D^{\bm w}_{\bm \Sigma} \; \gpdf{\bm z}{\bm \Sigma} & = \frac{\partial^{2 \|\bm w\|}}{\partial z_1^{\degree_1(\bm w)} \; \partial z_2^{\degree_2(\bm w)} \cdots \partial z_k^{\degree_k(\bm w)}} \; \gpdf{\bm z}{\bm \Sigma}.
\end{align*}
An inductive calculation shows that the ratio:
\begin{align*}
     \frac{1}{\gpdf{\bm z}{\bm \Sigma}}\; \frac{\partial^{2 \|\bm w\|}}{\partial z_1^{\degree_1(\bm w)} \; \partial z_2^{\degree_2(\bm w)} \cdots \partial z_k^{\degree_k(\bm w)}} \; \gpdf{\bm z}{\bm \Sigma},
\end{align*}
is a polynomial of degree $4 \|\bm w\|$ in the variables $z_1,z_2 \dots z_k, \{(\bm \Sigma^{-1})_{ij}\}_{i<j}$. Hence:
\begin{align*}
    &\left| \frac{1}{\gpdf{\bm z}{\bm \Sigma}}\; \frac{\partial^{2 \|\bm w\|}}{\partial z_1^{\degree_1(\bm w)} \; \partial z_2^{\degree_2(\bm w)} \cdots \partial z_k^{\degree_k(\bm w)}} \; \gpdf{\bm z}{\bm \Sigma}\right|  \leq \\ & \hspace{4cm}  C_{\|\bm w\|} \cdot ( 1 + \sum_{i < j} |(\bm \Sigma^{-1})_{ij}|^{4 \|\bm w\|} + \sum_{i=1}^k |z_i|^{4\|\bm w\|}),
\end{align*}
where $C_{\|\bm w\|}$ denotes a constant depending only on $\|\bm w\|$. Observing that:
\begin{align*}
    (\bm \Sigma^{-1})_{ij} & \leq \|\bm \Sigma^{-1}\|_{\op}  = \frac{1}{\lambda_{\min}(\bm \Sigma)} < \infty.
\end{align*}
This gives us:
\begin{align*}
      \left| \frac{1}{\gpdf{\bm z}{\bm \Sigma}}\; \frac{\partial^{2 \|\bm w\|}}{\partial z_1^{\degree_1(\bm w)} \; \partial z_2^{\degree_2(\bm w)} \cdots \partial z_k^{\degree_k(\bm w)}} \; \gpdf{\bm z}{\bm \Sigma}\right| & \leq C_{\|\bm w\|}  \left( 1 + \frac{k^2}{\lambda_{\min}^{4\|\bm w\|}(\bm \Sigma)} + \sum_{i=1}^k |z_i|^{4\|\bm w\|}\right).
\end{align*}
Substituting this estimate in \eqref{eq: taylors_thm} gives us:
\begin{align*}
    &\left|\gpdf{\bm z}{\bm \Sigma} -  \sum_{\bm w \in \weightedG{k}: \|\bm w\| \leq t} \frac{D^{\bm w}_{\bm \Sigma} \; \psi(\bm z; \bm I_k)}{\bm w !} \cdot \bm \Sigma^{\bm w}  \right|  \\& \hspace{2cm} \leq  C_{t,k} \cdot \left( 1 + \frac{k^2}{\lambda_{\min}^{4t+4}(\bm \Sigma_\gamma)} + \sum_{i=1}^k |z_i|^{4t+4}\right)\cdot \left( \max_{i \neq j} |\Sigma_{ij}| \right)^{t+1} \cdot \gpdf{\bm z}{\bm \Sigma_{\gamma}}.
\end{align*}
Note that $\lambda_{\min}(\bm \Sigma_\gamma) = \gamma + (1-\gamma) \lambda_{\min}(\bm \Sigma) \geq \min(1,\lambda_{\min}(\bm \Sigma))$. Hence,
\begin{align*}&\left|\gpdf{\bm z}{\bm \Sigma} -  \sum_{\bm w \in \weightedG{k}: \|\bm w\| \leq t} \frac{D^{\bm w}_{\bm \Sigma} \; \psi(\bm z; \bm I_k)}{\bm w !} \cdot \bm \Sigma^{\bm w}  \right|  \\& \hspace{1cm} \leq  C_{t,k} \cdot \left( 1 + \frac{k^2}{\min(\lambda_{\min}^{4t+4}(\bm \Sigma),1)} + \sum_{i=1}^k |z_i|^{4t+4}\right)\cdot \left( \max_{i \neq j} |\Sigma_{ij}| \right)^{t+1} \cdot \gpdf{\bm z}{\bm \Sigma_{\gamma}}.
\end{align*}
Using this expansion to compute the expectation of $\prod_{i=1}^k f_i(z_i)$ we obtain:
\begin{align*}
   \left| \E \left[ \prod_{i=1}^k f_i(z_i) \right] - \sum_{\substack{\bm w \in \weightedG{k}\\ \|\bm w\| \leq t}}   \left( \prod_{i=1}^k \hat{f}_i(\degree_i(\bm w)) \right) \cdot \frac{\bm \Sigma^{\bm w}}{\bm w!} \right| & \leq C \left(1 + \frac{1}{\lambda_{\min}^{4t+4}(\bm \Sigma)} \right)  \left( \max_{i \neq j} |\Sigma_{ij}| \right)^{t+1},
\end{align*}
where $C=C_{t,k,f_{1:k}}$ denotes a constant depending only on $t,k$ and the functions $f_{1:k}$.
In obtaining the above estimate we use the fact that since the functions $f_i$ have polynomial growth and marginally $z_i \sim \gauss{0}{1}$ under the measure $\gauss{\bm 0}{\bm \Sigma_{\gamma}}$ (since $(\Sigma_{\gamma})_{ii} = 1$) we have,
\begin{align*}
    \E_{\bm z \sim \gauss{\bm 0}{\bm \Sigma_\gamma}} \left[ |z_i|^{4t+4} \prod_{j=1}^k |f_j(z_j)| \right] & \leq \sum_{j=1}^k \E_{\bm z \sim \gauss{\bm 0}{\bm \Sigma_\gamma}} \left[ |z_i|^{4t+4} |f_j(z_j)|^k \right]  = C_{t,k,f_{1:k}} < \infty.
\end{align*}
\end{proof}

% We also version Proposition \ref{proposition: mehler} for complex Gaussians. The proof is analogous.

% \begin{prop} \label{proposition: mehler_complex} Let $f_1,f_2 \dots f_k: \C \rightarrow \R$ be $k$ arbitrary functions whose absolute value can be upper bounded by a polynomial. Consider a $k$ dimensional complex Gaussian vector $\bm z = \bm u + \i \bm v \in \C^k$ where $(\bm u, \bm v) \sim \gauss{\bm 0}{\bm \Sigma}$ is a 2k-dimensional real Gaussian vector  such that $\Sigma_{ii} = 1$ for all $i \in [2k]$.  
% Then,
% \begin{align*}
%   \left| \E \left[ \prod_{i=1}^k f_i(z_i) \right] - \sum_{\substack{\bm w \in \weightedG{2k}\\ \|\bm w\| \leq t}}   \left( \prod_{i=1}^k \hat{f}_i(\degree_i(\bm w),d_{i+k}(\bm w)) \right) \cdot \frac{\bm \Sigma^{\bm w}}{\bm w!} \right| & \leq C_{t,k, f_{1:k}} \left(1 + \frac{1}{\lambda_{\min}^{4t+4}(\bm \Sigma)} \right) \cdot \left( \max_{i \neq j} |\Sigma_{ij}| \right)^{t+1},
% \end{align*}
% where:
% \begin{align*}
%     \hat{f}_i(j,j^\prime) \explain{def}{=} \E f(Z + \i Z^\prime) H_j(Z) H_j^\prime(Z^\prime), \; Z, Z^\prime \explain{i.i.d.}{\sim} \gauss{0}{1}, 
% \end{align*}
% and the other notations are as in Proposition \ref{proposition: mehler}.
% \end{prop}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Derivation of Proposition \ref{prop: SE_rotationally_invariant}} \label{sec:appendix-SE-derivation}
In this section, we sketch how Proposition \ref{prop: SE_rotationally_invariant} can be derived by instantiating \citet[Theorem 1]{venkataramanan2021estimation} to our setup. Recall that the linearized AMP iterations are given by:
\begin{align}\label{eq:LAMP-recall}
     \hat{\bm z}^{(t+1)} &:= \left( \frac{1}{\kappa} \bm A \bm A^\UT - \bm I \right) \cdot  q_t(\bm Z) \cdot \hat{\bm z}^{(t)},
\end{align}
where, 
\begin{align} \label{eq:q-func-def}
    q_t(z) = \eta_t(|z|) - \E[\eta_t(|z|)],
\end{align} and $q_t(\bm Z) = \diag{q(z_1), q(z_2), \dotsc, q(z_m)}$ where $\bm z$ is the vector of signed measurements. Since we assume that the function $\eta$ is bounded and Lipschitz, $q_t$ is also a bounded Lipschitz function. 

We will obtain a state evolution result for iteration \eqref{eq:LAMP-recall}, we will relate it to an instance of a much more general class of approximate message passing algorithms studied in the work of \citet{venkataramanan2021estimation}. However, a minor difficulty is that the sensing matrix in our setup is obtained by picking $n$ columns of a $m \times m$ Haar matrix uniformly at random:
\begin{align*}
    \bm A = \bm H \bm P \bm S.
\end{align*}
In particular, $\bm A$ is left rotationally invariant but not right rotationally invariant, whereas the result in \citep{venkataramanan2021estimation} requires both left and right rotational invariance of the sensing matrix. The reason why this doesn't pose any difficulties is that it is easy to check that for any $\bm V \in \mathbb{O}(n)$, the sequence of iterates ${\hat{\bm z}}^{(t)}$ generated when the signal is $\bm x$ and the sensing matrix is $\bm A$ is identical to the sequence of iterates generated when the signal is $\bm V \bm x$ and the sensing matrix is $\bm A \bm V^\UT$. Hence by taking $\bm V \sim \unif{\mathbb{O}(n)}$, one obtains the desired right rotational invariance of the sensing ensemble. Next, we relate the iteration \eqref{eq:LAMP-recall} to the following iteration covered by the results in \citep{venkataramanan2021estimation}. We will closely follow the notation in \citep{venkataramanan2021estimation} for the convenience of the reader. Consider an algorithm that maintains two iterates $\bm x^{(t)}$ and $\bm r^{(t)}$ which are updated as follows:
\begin{subequations}\label{eq:venkat-AMP}
\begin{align}
    \bm x^{(t+1)} &= \bm A^\UT h_{t}(\bm r^{t}, \bm z) - \bm \epsilon^{(t+1)} \\
    \bm r^{(t+1)} &= \bm A  \bm x^{(t+1)} - \kappa \cdot h_t(\bm r^{(t)}, \bm z) - \bm \delta^{(t+1)}.
\end{align}
\end{subequations}
In the above display, $\kappa = n/m$ and the function $h_t : \R^2 \rightarrow \R$ acts entry-wise on the vectors $\bm r^{t}, \bm z$. We set $h_t(r,z) = r q_t(z)/\kappa$ to caliberate the iteration \eqref{eq:venkat-AMP} with \eqref{eq:LAMP-recall}. The vectors $\bm \epsilon^{(t+1)}$ and $\bm \delta^{(t+1)}$ are given by:
\begin{align*}
    \bm \epsilon^{(t)} & = \sum_{i=1}^{t-1}  \beta_{t,i} \cdot  \bm x^{(i)}, \\
    \bm \delta^{(t)} & = \sum_{i=1}^{t-1} \alpha_{t,i} \cdot h_{i-1}(\bm r^{(i-1)}) + (\alpha_{t,t} - \kappa) \cdot  h_{t-1}(\bm r^{(t-1)},\bm z),
\end{align*}
where the de-biasing coefficients $\alpha_{t,i}, \beta_{t,i}$ are as given in \citep[Equations 3.6-3.7]{venkataramanan2021estimation}. In order to relate iteration \eqref{eq:LAMP-recall} to the iteration \eqref{eq:venkat-AMP} we can combine the two iterations in \eqref{eq:venkat-AMP} to obtain:
\begin{align*}
    \bm r^{(t+1)} & = (\bm A \bm A^\UT - \kappa \bm I_{m}) \cdot h_t(\bm r^{(t)}, \bm z) - \bm A \bm \epsilon^{(t+1)} - \bm \delta^{(t+1)} \\
    & =  \left( \frac{1}{\kappa} \bm A \bm A^\UT - \bm I \right) \cdot  q_t(\bm Z) \cdot {\bm r}^{(t)} -  \bm A \bm \epsilon^{(t+1)} - \bm \delta^{(t+1)}. 
\end{align*}
We can now recursively control the error between the iterates $\| \bm r^{(t+1)} -  \hat{\bm z}^{(t+1)}\|_2$:
\begin{align}\label{eq:error-recursion}
    \| \bm r^{(t+1)} -  \hat{\bm z}^{(t+1)}\|_2 & \leq \frac{\|q_t\|_\infty}{\kappa} \cdot  \| \bm r^{(t)} -  \hat{\bm z}^{(t)}\|_2 + \|\bm \epsilon^{(t+1)}\|_2 + \|\bm \delta^{(t+1)}\|_2.
\end{align}
Using the formula for the de-biasing coefficients $\alpha_{t,i}, \beta_{t,i}$ are as given in \citep[Equations 3.6-3.7]{venkataramanan2021estimation} and the fact that:
\begin{align*}
    \frac{1}{m} \sum_{i=1}^m \partial_r h_t(r_i^{(t)},z_i) & = \frac{1}{m\kappa} \sum_{i=1}^m q_t(z_i) \explain{P}{\rightarrow} \frac{\E[q_t(Z)]}{\kappa} \explain{\eqref{eq:q-func-def}}{=} 0,
\end{align*}
we obtain that:
\begin{align*}
    \beta_{t,i} &\explain{P}{\rightarrow} 0\; \forall \; i \; \leq \; t-1, \\
    \alpha_{t,i} &\explain{P}{\rightarrow} 0\; \forall \; i \; \leq \; t-1, \\
     \alpha_{t,t} &\explain{P}{\rightarrow} \kappa.
\end{align*}
Which immediately yields for any $t \in \N$,
\begin{align*}
     \|\bm \epsilon^{(t)}\|^2_2/m \explain{P}{\rightarrow} 0, \; \|\bm \delta^{(t)}\|^2_2/m \explain{P}{\rightarrow} 0. 
\end{align*}
Combining this with \eqref{eq:error-recursion} gives us:
\begin{align*}
     \frac{\| \bm r^{(t+1)} -  \hat{\bm z}^{(t+1)}\|^2_2}{m} &\explain{P}{\rightarrow} 0.
\end{align*}
Consequently, the state evolution for the iteration $\bm r^{(t+1)}$ given in \citep[Theorem 1]{venkataramanan2021estimation} also holds for $\hat{\bm z}^{(t+1)}$, which gives us the claim of Proposition \ref{prop: SE_rotationally_invariant}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% APPENDIX-MISC%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Some Miscellaneous Facts}

\begin{fact}[Hanson-Wright Inequality \citep{rudelson2013hanson}] \label{fact: hanson_wright} Let $\bm x = (x_1, x_2 \dots,x_n) \in \R^n$ be a random vector with independent 1-subgaussian, zero mean components. Let $\bm A$ be an $n \times n$ matrix. Then, for every $t \geq 0$,
\begin{align*}
    \P \left( | \bm x^\UT \bm A \bm x - \E \bm x^\UT \bm A \bm x| > t \right) & \leq 2 \exp \left( - c \min \left( \frac{t^2}{\|\bm A\|_{\mathsf{Fr}}^2}, \frac{t}{\|\bm A\|_\op} \right) \right).
\end{align*}
\end{fact}


\begin{fact}[Gaussian Poincare Inequality] \label{fact: gaussian_poincare}Let $\bm x \sim \gauss{0}{\bm I_n}$. Then, for any $L$-Lipchitz function $f: \R^n \rightarrow \R$ we have,
\begin{align*}
    \var(f(\bm x)) & \leq L^2.
\end{align*}
\end{fact}

\begin{fact}[Moments of a Random Unit vector, Lemma 2.22 \& Proposition 2.5 of \citep{meckes2019random}] \label{fact: unit_vector_moments} Let $\bm x \sim \unif{\mathbb{S}_{n-1}}$. Let $i,j,k,\ell$ be distinct indices. Then:
\begin{align*}
    \E x_i^4 & = \frac{3}{n(n+2)}, \; \E x_i^2 x_j^2  = \frac{n+1}{n(n-1)(n+2)} \; \E x_i^3 x_j = 0 \; \E x_i x_j x_k^2 = 0, \; \E x_i x_j x_k x_l = 0.
\end{align*}
Furthermore, there exists a universal constant $C$ such that, for any $t \in \N$:
\begin{align*}
    \E |x_i|^t & \leq \left( \frac{Ct}{m} \right)^{\frac{t}{2}}.
\end{align*}
\end{fact}

\begin{fact}[Concentration on the Sphere, \citet{ball1997elementary}] \label{fact: concentration_sphere} Let $\bm x \sim \unif{\mathbb{S}_{n-1}}$. Then
\begin{align*}
    \P \left( |x_1| \geq \epsilon \right) & \leq 2 e^{-n \epsilon^2/2}.
\end{align*}
\end{fact}

\begin{fact}[$\ell_\infty$ norm of a random unit vector] \label{fact: infty_norm_uniform_unit}  $\bm x \sim \unif{\mathbb{S}_{n-1}}$. Then
\begin{align*}
    \E \|\bm x\|_\infty^t & \leq   \left( \frac{C  \log(n) }{n} \right)^{\frac{t}{2}},
\end{align*}
for a universal constant $C$.
\end{fact}
\begin{proof}
For a random unit vector we can control $\E \|\bm x\|_\infty^t$ as follows. Let $q \in \N$ be a parameter to be set suitably. Then,
\begin{align*}
    \E \|\bm x\|_\infty^t & = \left( \E \|\bm x\|_\infty^{qt} \right)^{\frac{1}{q}} \\
    & \leq \left( \sum_{i=1}^n \E |x_i|^{qt} \right)^{\frac{1}{q}} \\
    & \explain{(a)}{=} \left( n \E |x_1|^{qt} \right)^{\frac{1}{q}} \\
    & \explain{(b)}{=} n^{\frac{1}{q}} \cdot q^{\frac{t}{2}} \cdot  \left( \frac{C t}{n} \right)^{\frac{t}{2}} \\
    & \explain{(c)}{\leq} e^t \cdot (2 \log(n))^{\frac{t}{2}} \cdot  \left( \frac{C  }{n} \right)^{\frac{t}{2}}.
\end{align*}
In the step marked (a) we used the fact that the coordinates of a random unit vector are exchangeable, in (b) we used the fact that $u_1$ is $C/m$-subgaussian (see Fact \ref{fact: concentration_sphere}) and in (c) we set $q = \lfloor \frac{2\log(n)}{t} \rfloor$.
\end{proof}
\begin{fact}[Poincare Inequality for Haar Measure, \citet{gromov1983topological}]  \label{fact: poincare_haar}Consider the following setups:
\begin{enumerate}
    \item Let $\bm O \sim \unif{\O(m)}$ and $f: \R^{m \times m} \rightarrow \R$ be a function such that:
    \begin{align}
        f(\bm O) & = f(\bm O \bm D), \; \bm D = \diag{1,1,1, \dots, 1, \mathsf{sign}(\det(\bm O))},  \label{eq: condition_poincare}
    \end{align}
    then,
    \begin{align*}
        \var(f(\bm O )) & \leq \frac{8}{m} \cdot \E \|\nabla f(\bm O)\|_\fr^2.
    \end{align*}
    for any $m \geq 4$.
    \item  Let $\bm O \sim \unif{\mathbb{U}(m)}$ and $f: \mathbb{C}^{m \times m} \rightarrow \R$. Then,
    \begin{align*}
        \var(f(\bm O )) & \leq \frac{8}{m} \cdot \E \|\nabla f(\bm O)\|_\fr^2.
    \end{align*}
\end{enumerate}
\end{fact}
\begin{proof} This result is due to \citet{gromov1983topological}. Our reference for these inequalities was the book of \citet{meckes2019random}. Theorem 5.16 of \citeauthor{meckes2019random} shows that Haar measures on $\mathbb{SO}(m), \mathbb{U}(m)$ satisfy Log-sobolev inequality with constant $8/m$. It is well known that Log-Sobolev Inequality implies the Poincare Inequality (see for e.g.  Lemma 8.12 in \citet{van2014probability}). Note that, in the real case we only obtain the Poincare inequality for the Haar measure on $\mathbb{SO}(m)$, condition \eqref{eq: condition_poincare} ensures the result still holds for  $\bm O \sim \unif{\O(m)}$.
\end{proof}

\begin{fact}[Continuity of Matrix Square Root {\citep[Lemma 2.2]{schmitt1992perturbation}}] \label{fact: matrix_sqrt} For any two symmetric positive semi-definite matrices $\bm M_1, \bm M_2$ we have,
\begin{align*}
    \|{\bm M}_1^{\frac{1}{2}} - \bm M_2^{\frac{1}{2}} \|_{\op} & \leq \frac{ \|{\bm M}_1 - \bm M_2 \|_{\op}}{\sqrt{\lambda_{\min}(\bm M_1)}}.
\end{align*}
\end{fact}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> arxiv final/packages.tex <==
% math packeges
\usepackage{amsthm,amsfonts,amsmath, amssymb,dsfont,color, multirow}
\usepackage{commath,enumerate, mathtools,float,graphicx}


%rishabh added these
\usepackage{bm,thmtools}
\usepackage{hyperref}
\usepackage[numbers]{natbib}
%\usepackage[inline]{showlabels}
\usepackage{mathrsfs,soul}



%\theoremstyle{theorem} % was generating warning -- Rishabh
\newtheorem{thm}{{Theorem}}[]
\newtheorem{coro}{\textbf{Corollary}}[]
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{exmp}{Example}
\newtheorem{rem}{Remark}
\newtheorem{defn}{Definition}
\newtheorem{fact}{Fact}


%Other packages
%\usepackage{cite}
\usepackage{balance}
\usepackage[T1]{fontenc}

% Graphical packages
\usepackage{subcaption, multirow} 
\usepackage{makecell}


% Matrix/Vector notation
\newcommand{\mvec}[1]{{\boldsymbol #1}}
\newcommand{\xv}{\mvec{x}}
\newcommand{\cv}{\mvec{c}}
\newcommand{\yv}{\mvec{y}}
\newcommand{\zv}{\mvec{z}}
%\newcommand{\diag}[1]{{\rm diag}\intoo{#1}} I have redefined it with the same notation -- Rishabh


% Other symbols
\def\A{\mathcal{A}}
\def\F{\mathcal{F}}
\def\H{\mathcal{H}}
\def\J{\mathcal{J}}
\def\S{\mathcal{S}}
%\def\N{\mathcal{N}}  %% Use \gauss{mean}{covariance}
%\def\P{\mathcal{P}} %% This clashes with one of my commands -- Rishabh
%\def\E{\mathcal{E}} %% This clashes with one of my commands -- Rishabh
\def\D{\mathcal{D}}
%\def\C{\mathcal{C}} %%this clashes with one of my commands -- Rishabh
%\def\N{\mathcal{N}} %%this clashes with one of my commands -- Rishabh
\def\X{\mathcal{X}}
\def\T{\mathcal{T}}
\def\Q{\mathcal{Q}}
\def\rme{{\rm e}}

% Probability commands
\newcommand{\p}[2][{}]{\mathbb{P}_{#1} \intoo{#2}}
\newcommand{\e}[2][{}]{\mathbb{E}_{#1} \sbr{#2}}
\newcommand{\expp}[1]{\exp \intoo{#1}}

% Norms
\newcommand{\normp}[1]{\norm{#1}_p}

% Operators
\newcommand{\define}{\triangleq}


% Beamer Setting -- Creates error with one of my packages -- Rishabh
%\usepackage[absolute,overlay]{textpos}
%\usepackage{bibentry}
%\usepackage[sort&compress]{natbib}


%Rishabh uses these macros

\newcommand{\mr}{\mathrm}
\newcommand{\UH}{\mathsf{H}}   %% upright H
\newcommand{\UT}{\mathsf{T}}   %% upright T
\renewcommand{\Re}{\mr{Re}}  
\renewcommand{\Im}{\mr{Im}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\hatE}{\hat{\E}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}} %% Use \gauss{mean}{covariance}
\newcommand{\R}{\mathbb{R}}
\renewcommand{\O}{\mathbb{O}}
\newcommand{\W}{\mathbb{N}_0}
\newcommand{\Tr}{\mathsf{Tr}}
\newcommand{\tr}{\mathsf{tr}}
\newcommand{\rComment}[1]{{\color{blue}{#1}}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\gauss}[2]{\mathcal{N}\left( #1,#2 \right)}
\newcommand{\cgauss}[2]{\mathcal{CN}\left( #1,#2 \right)}
\newcommand{\explain}[2]{\overset{\text{\tiny{#1}}}{#2}}
\newcommand{\diag}[1]{\text{Diag}\left(#1\right)}
\newcommand{\Arg}{\mathsf{Arg}}
\newcommand{\Spec}[1]{\mathsf{Spec}\left(#1\right)}
\newcommand{\Indicator}[1]{\mathbb{I}_ {#1}}
\newcommand{\gpdf}[2]{\psi(#1;#2)}
\newcommand{\ip}[2]{\langle {#1}, {#2} \rangle}
\renewcommand{\vec}[1]{\mathsf{Vec} \left( #1 \right)}
\renewcommand{\i}{\mathrm{i}}
\newcommand{\unif}[1]{\text{Unif} \left( #1 \right)}
\newcommand{\barB}{\overline{\bm B}}
\newcommand{\bern}{\mathsf{Bern}}
\newcommand{\altprod}{\mathcal{\bm A}}
\renewcommand{\part}[2]{\mathcal{P}_{#1}(#2)}
\newcommand{\blocks}{\mathcal{V}}
\newcommand{\cset}[1]{\mathcal{C}(#1)}
\newcommand{\op}{\mathsf{op}}
\newcommand{\trim}{\mathcal{T}}
\newcommand{\weightedG}[1]{\mathcal{G}(#1)}
\newcommand{\weightedGnum}[2]{\mathcal{G}_{\mathsf{#2}}(#1)}
\newcommand{\degree}{\mathsf{d}}
\newcommand{\matmom}[4]{\mathcal{M}(#1,#2,#3,#4)}
\newcommand{\limmom}[2]{{\mu}(#1,#2)}
\DeclareMathOperator*{\plim}{p-lim}
\newcommand{\bnomdistr}[2]{\mathsf{Binom}(#1,#2)}
\newcommand{\fr}{\mathsf{Fr}}
\DeclareMathOperator*{\var}{Var}
\DeclareMathOperator*{\polylog}{polylog}
\newcommand{\singleblks}[1]{\mathscr{S}(#1)}
\newcommand{\firstblk}[1]{\mathscr{F}(#1)}
\newcommand{\centerblk}[2]{\mathscr{C}_{#1}(#2)}
\newcommand{\fblknum}[2]{\mathscr{F}_{#1}(#2)}
\newcommand{\lblknum}[2]{\mathscr{L}_{#1}(#2)}
\newcommand{\firstfnc}{\mathscr{F}}
\newcommand{\ffncnum}[1]{{\mathscr{F}_{#1}}}
\newcommand{\lfncnum}[1]{{\mathscr{L}_{#1}}}
\newcommand{\lastfnc}{\mathscr{L}}
\newcommand{\centerfnc}[1]{{\mathscr{C}_{#1}}}
\newcommand{\lastblk}[1]{\mathscr{L}(#1)}
\newcommand{\tbd}{\frac{1}{4}}
\newcommand{\labelling}[1]{\mathcal{L}_{\mathsf{#1}}}
\newcommand{\dlgraph}{\bm{\ell}_{k+1}^{\otimes 2}}
\newcommand{\coeff}{g}
\newcommand{\Coeff}{G}
\renewcommand{\bar}{\overline}



%Milad uses these

\newcommand{\barb}{\overline{\bm b}}
\newcommand{\hatb}{\hat{\bm b}}
% \newcommand{\milad}[1]{\textcolor{red}{#1}}
% \newcommand{\red}[1]{\textcolor{red}{#1}}
% \newcommand{\rishabh}[1]{\textcolor{blue}{#1}}
\newcommand{\milad}[1]{{#1}}
\newcommand{\rishabh}[1]{{#1}}
